Vector Space Over Division Ring

A system of linear equations over a skew field has properties similar to properties of a system of linear equations over a field. Even noncommutativity of a product creates a new picture the properties of system of linear equations and of vector space over skew-field have a close relationship.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem
{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление $\mathfrak{F}$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:q-alg/1004.3007} (2010)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-rcd форма
   {$1$-\rcd форма}%
   {1-rcd form, vector spaces}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%3%A%a b-CR квазидетерминант
   {$(^a_b)$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%581%A%Arc  линейно зависимые векторы
   {$A\RCstar$\Hyph  линейно зависимые векторы}%
   {linearly dependent, A vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%580%A%Arc линейно независимые векторы
   {$A\RCstar$\Hyph линейно независимые векторы}%
   {linearly independent, A vector space}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%13%C%crd производная Гато отображения \Vector f D-векторного пространства \Vector V в D-векторное пространство \Vector W
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%20%D%Drc  линейно зависимые векторные поля
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%111%D%drc аффинный базис
   {\drc аффинный базис}%
   {drc affine basis, division ring}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%16%D%drc базис векторного пространства r строк
   {\drc базис векторного пространства \subs строк}%
   {drc basis, r rows vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%30%D%drc вектор-функция
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index%33%D%Drc линейно независимые векторные поля
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%38%D%drc производная Гато отображения \Vector f D- векторного пространства \Vector V в D- векторное пространство \Vector W
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%42%D%Dstar компонента координат вектора \Vector r
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%25%D%rcd базис в векторном пространстве c строк
   {\rcd базис в векторном пространстве \sups строк}%
   {rcd basis, c rows vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%49%R%drc базис, дуальный rcd базису в векторном пространстве
   {\drc базис, дуальный \rcd базису в векторном пространстве}%
   {basis dual to basis, rcd vector space}%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главный минор
   {\RC главный минор}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%21%R%rcd  линейно зависимые векторы
   {\rcd  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%24%R%rcd базис в векторном пространстве
   {\rcd базис в векторном пространстве}%
   {rcd basis, vector space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%34%R%rcd линейно независимые векторы
   {\rcd линейно независимые векторы}%
   {linearly independent, vector space}%
\Index%35%R%rcd линейное отображение векторных пространств
   {\rcd линейное отображение векторных пространств}%
   {rcd linear map of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%71%R%Rstar- модуль
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index%77%S%Dstar- произведением rcd линейного отображения A на скаляр
   {$D\star$\Hyph произведением \rcd линейного отображения $A$ на скаляр}%
   {Dstar product of rcd linear map over scalar}%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%586%S%star A- product of Astar linear map over scalar
   {$\star A$\Hyph произведением $A\star$\Hyph линейного отображения на скаляр}%
   {starA product of Astar linear map over scalar}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%75%S%starD компонента координат вектора \Vector r
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%88%T%Tstar- линейная комбинация векторов
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления F алгебры
   {автоморфизм представления $\mathfrak{F}$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%96%А%аддитивное отображение D- векторных пространств
   {аддитивное отображение $D$\Hyph векторных пространств}%
   {additive map of D vector spaces}%
\Index%98%А%аддитивное отображение тела, порождённое отображением G
   {аддитивное отображение тела, порождённое отображением $G$}%
   {additive map generated by map, division ring}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление лупы в многообразии базисов
   {активное представление лупы $\mathfrak A(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%616%А%ассоциатор R алгебры
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%117%Б%базовый вектор представления группы Ли
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%121%Б%бесконечно малый генератор
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index%123%В%вектор Килинга второго рода
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%130%В%вырожденное аддитивное отображение D- векторного пространства
   {вырожденное аддитивное отображение $D$\Hyph векторного пространства}%
   {singular additive map, D vector space}%
\Index%131%В%вырожденное аддитивное отображение тела
   {вырожденное аддитивное отображение тела}%
   {singular additive map, division ring}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\mathcal{E}$}%
   {Cartesian power n of bundle E}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%156%Д%дифференциал Гато второго порядка отображения \Vector f
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Index%155%Д%дифференциал Гато второго порядка отображения f
   {дифференциал Гато второго порядка отображения $f$}%
   {Gateaux differential of Second Order, division ring}%
\Index%632%Д%дифференциал Гато второго порядка отображения f алгебры
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Index%157%Д%дифференциал Гато отображения \Vector f нормированного D- векторного пространства V в нормированное D- векторное пространство W
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Index%158%Д%дифференциал Гато отображения f
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Index%628%Д%дифференциал Гато отображения алгебры
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\SetIndexSpace%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор R алгебры
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%192%К%компонента линейного отображения D- векторного пространчства
   {компонента линейного отображения $D$\Hyph векторного пространчства}%
   {component of linear map, D vector space}%
\Index%193%К%компонента линейного отображения f тела
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Index%194%К%компонента полиаддитивного отображения \Vector A
   {компонента полиаддитивного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Index%195%К%компонента полилинейного отображения тела
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Index%196%К%компонента производной Гато второго порядка отображения \Vector f(\Vector x)
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Index%633%К%компонента производной Гато второго порядка отображения f(x) алгебры
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Index%197%К%компонента производной Гато второго порядка отображения тела
   {компонента производной Гато второго порядка отображения тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Index%199%К%компонента производной Гато отображения \Vector f(\Vector x)
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Index%198%К%компонента производной Гато отображения f(x)
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Index%629%К%компонента производной Гато отображения f(x) алгебры
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%204%К%координатная матрица вектора в rcd базисе
   {координатная матрица вектора в \rcd базисе}%
   {coordinate matrix of vector in rcd basis}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов в векторном пространстве dcr строк
   {координатная матрица множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\Index%207%К%координатная матрица множества векторов в векторном пространстве rcd строк
   {координатная матрица множества векторов в векторном пространстве \rcd строк}%
   {coordinate matrix of set of vectors, rcd vector space}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%323%К%координаты автоморфизма представления
   {координаты автоморфизма представления}%
   {coordinates of automorphism of representation}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора в rcd базисе
   {координаты вектора в \rcd базисе}%
   {coordinates of vector in rcd basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%222%К%координаты множества векторов в dcr векторном пространстве
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index%223%К%координаты множества векторов в rcd векторном пространстве
   {координаты множества векторов в \rcd векторном пространстве}%
   {coordinates of set of vectors, rcd vector space}%
\Index%571%К%координаты пассивного отображения многообразия базисов представления
   {координаты пассивного отображения многообразия базисов представления}%
   {coordinates of passive map of basis manifold of representation}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%558%К%координаты элемента относительно множества
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%608%Л%линейное отображение  R_1 модуля в R_2 модуль
   {линейное отображение  $R_1$\Hyph модуля $A_1$ в $R_2$\Hyph модуль $A_2$}%
   {linear mapping of R_1 module into R_2 module}%
\Index%241%Л%линейное отображение D- векторных пространств
   {линейное отображение $D$\Hyph векторных пространств}%
   {linear map, vector space}%
\Index%242%Л%линейное отображение D- векторных пространств над полем F
   {линейное отображение $D$\Hyph векторных пространств над полем $F$}%
   {linear map over field, vector space}%
\Index%610%Л%линейное отображение R алгебры в R алгебру
   {линейное отображение $R$\Hyph алгебры $A_1$ в $R$\Hyph алгебру $A_2$}%
   {linear mapping of R algebras}%
\Index%613%Л%линейное отображение R модуля в R модуль
   {линейное отображение $R$\Hyph модуля $A_1$ в $R$\Hyph модуль $A_2$}%
   {linear mapping of R modules}%
\Index%243%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map, division ring}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear mapping of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\Index%568%Л%лупа автоморфизмов представления
   {лупа автоморфизмов представления}%
   {loop of automorphisms of representation}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%584%М%матрица Astar линейного отображения
   {матрица $A\star$\Hyph линейного отображения}%
   {matrix of Astar linear map}%
\Index%251%М%матрица rcd линейного отображения
   {матрица \rcd линейного отображения}%
   {matrix of rcd linear map}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов H алгебры
   {матрица эндоморфизмов $\mathfrak{H}$\Hyph алгебры}%
   {matrix of endomorphisms of H algebra}%
\Index%527%М%матрица Якоби Гато отображения D- векторного пространства
   {матрица Якоби\Hyph Гато отображения $D$\Hyph векторного пространства}%
   {Jacobi Gateaux matrix of map, D vector space}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%647%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие drc базисов аффинного пространства
   {многообразие \drc базисов аффинного пространства}%
   {drc Basis Manifold, Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index%270%Н%направление в D- векторном пространстве \Vector V над полем P
   {направление в $D$\Hyph векторном пространстве $\Vector V$ над полем $P$}%
   {direction over field, D vector space}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%313%Н%непрерывная функция над алгебро1
   {непрерывная функция над $D$\Hyph алгебро1}%
   {continuous function, algebra}%
\Index%280%Н%непрерывная функция тела
   {непрерывная функция тела}%
   {continuous function, division ring}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%648%Н%норма на D- алгебре
   {норма на $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%285%Н%норма отображения  тела
   {норма отображения  тела}%
   {norm of map, division ring}%
\Index%286%Н%норма отображения \Vector A нормированного D-векторного пространства
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Index%314%Н%норма отображения в D- алгебру
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Index%649%Н%нормированная D- алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%287%Н%нормированное D- векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\SetIndexSpace%
\Index%289%О%образующая аддитивного отображения
   {образующая аддитивного отображения}%
   {generator of additive map, division ring}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормальный базис
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормальный базис
   {ортонормальный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированый базис в пространстве Минковского
   {ортонормированый базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%310%О%отображение D- векторного пространства, мультипликативное над полем
   {отображение $D$\Hyph векторного пространства, мультипликативное над полем}%
   {map multiplicative over field, D vector space}%
\Index%311%О%отображение D- векторного пространства, проективное над полем
   {отображение $D$\Hyph векторного пространства, проективное над полем}%
   {map projective over field, D vector space}%
\Index%312%О%отображение колец R_1, ..., R_n, полилинейное над коммутативным кольцом P
   {отображение полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%342%П%полиаддитивное отображение (n)-D-векторных пространств
   {полиаддитивное отображение $(n)$\hyph $D$\hyph векторных пространств}%
   {polyadditive map of D vector spaces}%
\Index%343%П%полиаддитивное отображение колец
   {полиаддитивное отображение колец}%
   {polyadditive map of rings}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric, division ring}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%609%П%полилинейное отображение алгебр
   {полилинейное отображение алгебр}%
   {polylinear map of algebras}%
\Index%346%П%полилинейное отображение колец
   {полилинейное отображение колец}%
   {polylinear map of rings}%
\Index%621%П%полилинейное отображение модулей
   {полилинейное отображение модулей}%
   {polylinear map of modules}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric, division ring}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%644%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%351%П%последовательность Коши в нормированное теле
   {последовательность Коши в нормированное теле}%
   {Cauchy sequence, valued division ring}%
\Index%271%П%последовательность Коши в нормированном алгебре
   {последовательность Коши в нормированном алгебрае}%
   {Cauchy sequence, normed algebra}%
\Index%643%П%последовательность Коши в нормированном кольце
   {последовательность Коши в нормированном кольце}%
   {Cauchy sequence, normed ring}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%650%П%предел последовательности в нормированной алгебре
   {предел последовательности в нормированной алгебре}%
   {limit of sequence, normed algebra}%
\Index%651%П%предел последовательности в нормированном кольце
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Index%364%П%предел последовательности в нормированном теле
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%384%П%принцип инвариантности
   {принцип инвариантности}%
   {invariance principle}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\mathcal{E}$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка отображения f
   {производная Гато второго порядка отображения $f$}%
   {Gateaux derivative of Second Order, division ring}%
\Index%626%П%производная Гато второго порядка отображения алгебры
   {производная Гато второго порядка отображения алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Index%397%П%производная Гато отображения f
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Index%398%П%производная Гато отображения Vector f нормированого D- векторного пространства Vector V в нормированное D- векторное пространство Vector W
   {производная Гато отображения $\Vector f$ нормированого $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Index%627%П%производная Гато отображения алгебры
   {производная Гато отображения алгебры}%
   {Gateaux derivative of map, algebra}%
\Index%399%П%производная Гато порядка n отображения \Vector f
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Index%634%П%производная Гато порядка n отображения f алгебры
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Index%400%П%производная Гато порядка n отображения f тела
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%645%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%453%С%смешанная частная производная Гато отображения f^j по переменным v^i, v^j
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%456%С%стандартная F- компонента аддитивного отображения f
   {стандартная $F$\Hyph компонента аддитивного отображения $f$}%
   {standard component of additive map, division ring}%
\Index%458%С%стандартная компонента дифференциала Гато отображения f
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Index%459%С%стандартная компонента квадратичного отображения f над полем F
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Index%460%С%стандартная компонента линейного отображения тела
   {стандартная компонента линейного отображения тела}%
   {standard component of linear map, division ring}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения f тела
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Index%630%С%стандартная компонента производной Гато отображения f
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%
\Index%574%С%стандартная компонента тензора в тензорном произведении алгебр
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Index%464%С%стандартное F- представление аддитивного отображения тела
   {стандартное $F$\Hyph представление аддитивного отображения тела}%
   {additive map, standard representation, division ring}%
\Index%465%С%стандартное представление дифференциала Гато отображения тела над полем F
   {стандартное представление дифференциала Гато отображения тела над полем $F$}%
   {Gateaux differential, standard representation, division ring}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%467%С%стандартное представление линейного отображения тела
   {стандартное представление линейного отображения тела}%
   {linear map, standard representation, division ring}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения тела
   {стандартное представление полилинейного отображения тела}%
   {polylinear map, standard representation, division ring}%
\Index%631%С%стандартное представление производной Гато отображения над алгеброй
   {стандартное представление производной Гато отображения над алгеброй}%
   {Gateaux derivative, standard representation, algebra}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%618%С%структурные константы алгебры над кольцом
   {структурные константы алгебры $A$ над кольцом $R$}%
   {structural constants of algebra}%
\Index%473%С%структурные константы тела D над полем F
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%475%С%сумма rcd линейных отображений
   {сумма \rcd линейных отображений}%
   {sum of rcd linear maps, rcd vector spaces}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%646%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%487%Т%топологическое drc векторное пространство
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%493%У%уравнение Килинга
   {уравнение Килинга}%
   {Killing equation}%
\Index%494%У%уравнение Килинга второго рода
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%500%Ф%фундаментальная последовательность в нормированное теле
   {фундаментальная последовательность в нормированное теле}%
   {fundamental sequence, valued division ring}%
\Index%652%Ф%фундаментальная последовательность в нормированном алгебре
   {фундаментальная последовательность в нормированном алгебре}%
   {fundamental sequence, normed algebra}%
\Index%642%Ф%фундаментальная последовательность в нормированном кольце
   {фундаментальная последовательность в нормированном кольце}%
   {fundamental sequence, normed ring}%
\Index%502%Ф%функция \gi n D- значных переменных
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index%501%Ф%функция D- векторного пространства V в D- векторное пространство W, дифференцируемая по Гато
   {функция $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector W$, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, D vector space}%
\Index%625%Ф%функция алгебры, дифференцируемая по Гато
   {функция алгебры, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, algebra}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%505%Ф%функция тела, дифференцируемая по Гато
   {функция тела, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, division ring}%
\Index%506%Ф%функция, непрерывная по совокупности аргументов
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%510%Ч%частная crd производная Гато отображения fb по переменной xa
   {частная \crd производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial crd derivative of map with respect to variable, D vector space}%
\Index%511%Ч%частная drc производная Гато отображения f^b по переменной x^a
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато отображения f^j по переменной v^i
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Index%513%Ч%частное аддитивное отображение переменной v^i
   {частное аддитивное отображение переменной $v^i$}%
   {partial additive map of variable}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления F алгебры
   {эндоморфизм представления $\mathfrak{F}$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%324%Э%эффективная башня Tstar- представлений
   {эффективная башня \Ts представлений}%
   {effective tower of representations}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%522%Я%ядро аддитивного отображения D- векторного пространства
   {ядро аддитивного отображения $D$\Hyph векторного пространства}%
   {kernel of additive map, D vector space}%
\Index%523%Я%ядро аддитивного отображения тела
   {ядро аддитивного отображения тела}%
   {kernel of additive map, division ring}%
\Index%619%Я%ядро алгебры
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%

\CloseIndex


==> Rcd.Morphism.Russian.tex <==
%auto-ignore
\input{Rcd.Morphism}

\section{\texorpdfstring{$\RCstar D$}{Rcd}\hyph линейное отображение векторных пространств}
\label{section: Linear Map of Vector Spaces}

\begin{definition}
\label{definition: rcs rct linear map of vector spaces}
Пусть $\Vector V$ - $\RCstar S$\Hyph векторное пространство.
Пусть $\Vector U$ - $\RCstar T$\Hyph векторное пространство.
Мы будем называть морфизм
\[
\xymatrix{
f:S\ar[r]&T&\Vector A:\Vector V\ar[r]&\Vector U
}
\]
\Ts представлений тела в абелевой группе
\AddIndex{\StarST линейным отображением векторных пространств}
{rcs rct linear map of vector spaces}.
\qed
\end{definition}

Согласно теореме
\ref{theorem: decompositions of morphism of representations}
при изучении \StarST линейного отображения
мы можем ограничиться случаем $S=T$.

\begin{definition}
\label{definition: rcd linear map of vector spaces}
Пусть $\Vector V$ и
$\Vector W$ - \rcd векторные пространства.
Мы будем называть отображение
\ShowEq{rcd linear map of vector spaces}
\AddIndex{\rcd линейным отображением векторных пространств}
{rcd linear map of vector spaces},
если\footnote{Выражение
\ShowEq{rcd linear map of vector spaces, product on scalar, 1}
означает выражение
\ShowEq{rcd linear map of vector spaces, product on scalar, 2}
}
\ShowEq{rcd linear map of vector spaces, product on scalar}
для любых
\ShowEq{product on scalar, 1}
\qed
\end{definition}

\begin{theorem}
\label{theorem: rcd linear map of rcd vector space}
Пусть
\ShowEq{rcd vector space Basis f}
\rcd базис в векторном пространстве $\Vector V$
и
\ShowEq{rcd vector space Basis e}
\rcd базис в векторном пространстве $\Vector U$.
Тогда \rcd линейное отображение \EqRef{rcd linear map of vector spaces}
векторных пространств имеет представление
\ShowEq{rcd linear map of vector spaces, presentation}
относительно заданных базисов. Здесь
\begin{itemize}
\item $a$ - координатная матрица вектора
$\Vector a$ относительно \rcd базиса $\Basis f$
\item $b$ - координатная матрица вектора
$$\Vector b=\Vector A(\Vector a)$$ относительно \rcd базиса $\Basis e$
\item $A$ - координатная матрица множества векторов
\ShowEq{Vector A(f)}
в \rcd базисе $\Basis e$, которую мы будем называть
\AddIndex{матрицей \rcd линейного отображения}{matrix of rcd linear map}
относительно базисов $\Basis f$ и $\Basis e$
\end{itemize}
\end{theorem}
\begin{proof}
Вектор $\Vector a\in \Vector V$ имеет разложение
\ShowEq{eq: rcd linear map, 1}
относительно \rcd базиса $\Basis f$.
Вектор $\Vector{b}=f(\Vector a)\in \Vector U$ имеет разложение
\ShowEq{rcd linear map, 2}
относительно \rcd базиса $\Basis e$.

Так кaк $\Vector A$ - \rcd линейное отображение, то на основании
\EqRef{rcd linear map of vector spaces, product on scalar} следует,
что
\ShowEq{rcd linear map, 3}
\ShowEq{rcd linear map, 3i}
также вектор векторного пространства $\Vector U$ и имеет
разложение
\RcdMap{rcd linear map, 4}
относительно базиса $\Basis e$.
Комбинируя \EqRef{rcd linear map, 3}
и \EqRef{rcd linear map, 4}, мы получаем
\ShowEq{rcd linear map, 5}
\EqRef{rcd linear map of vector spaces, presentation}  следует
из сравнения \EqRef{rcd linear map, 2}
и \EqRef{rcd linear map, 5} и
теоремы \xRef{0701.238}{theorem: expansion relative basis, vector space}.
\end{proof}

На основании теоремы \ref{theorem: rcd linear map of rcd vector space}
мы идентифицируем \rcd линейное отображение \EqRef{rcd linear map of vector spaces}
векторных пространств и
матрицу его представления \EqRef{rcd linear map of vector spaces, presentation}.

\begin{theorem}
\label{theorem: product of rcd linear maps, vector spaces}
Пусть
\ShowEq{rcd vector space Basis f}
\rcd базис в векторном пространстве $\Vector V$,
\ShowEq{rcd vector space Basis e}
\rcd базис в векторном пространстве $\Vector U$,
и
\ShowEq{rcd vector space Basis g}
\rcd базис в векторном пространстве $\Vector W$.
Предположим, что мы имеем коммутативную диаграмму отображений
\[
\xymatrix{
\Vector V\ar[rr]^{\Vector C}\ar[dr]^{\Vector A} & & \Vector W\\
&\Vector U\ar[ur]^{\Vector B} &
}
\]
где \rcd линейное отображение $\Vector A$ имеет представление
\ShowEq{product of rcd linear maps, A}
относительно заданных базисов
и \rcd линейное отображение $\Vector B$ имеет представление
\ShowEq{product of rcd linear maps, B}
относительно заданных базисов.
Тогда отображение $\Vector C$ является \rcd линейным и имеет представление
\ShowEq{product of rcd linear maps, C}
относительно заданных базисов.
\end{theorem}
\begin{proof}
Отображение $\Vector C$ является \rcd линейным, так как
\ShowEq{product of rcd linear maps, vector spaces}
Равенство
\EqRef{product of rcd linear maps, C}
следует из подстановки
\EqRef{product of rcd linear maps, A}
в \EqRef{product of rcd linear maps, B}.
\end{proof}

Записывая \rcd линейное отображение в форме \RC произведения, мы можем переписать
\EqRef{rcd linear map of vector spaces, product on scalar} в виде
\ShowEq{rcd linear map of vector spaces, product on scalar, image}
Утверждение теоремы
\ref{theorem: product of rcd linear maps, vector spaces}
мы можем записать в виде
\ShowEq{product of rcd linear maps, vector spaces, image}
Равенства
\EqRef{rcd linear map of vector spaces, product on scalar, image} и
\EqRef{product of rcd linear maps, vector spaces, image}
представляют собой
\AddIndex{закон ассоциативности для \rcd линейных отображений векторных пространств}
{associative law for rcd linear maps of vector spaces}.
Это позволяет нам писать подобные выражения не пользуясь скобками.

Равенство \EqRef{rcd linear map of vector spaces, presentation}
является координатной записью \rcd линейного отображения.
На основе теоремы \ref{theorem: rcd linear map of rcd vector space}
бескоординатная запись также может быть представлена с помощью \RC произведения
\ShowEq{rcd linear map of vector spaces, presentation, 5}
Если подставить равенство
\EqRef{rcd linear map of vector spaces, presentation, 5} в теорему
\ref{theorem: product of rcd linear maps, vector spaces},
то мы получим цепочку равенств
\ShowEq{rcd linear map, 6}

\begin{remark}
\label{remark: drc linear map}
На примере \rcd линейных отображений легко видеть
насколько теорема 
\ref{theorem: decompositions of morphism of representations}
облегчает наши рассуждения при изучении морфизма \Ts представлений
$\Omega$\Hyph алгебры.
Договоримся в рамках этого замечания
теорию \rcd линейных отображений называть сокращённой теорией,
а теорию, излагаемую в этом замечании, называть расширенной теорией.

Пусть $\Vector V$ - $\RCstar S$\Hyph векторное пространство.
Пусть $\Vector U$ - $\RCstar T$\Hyph векторное пространство.
Пусть
\ShowEq{rcs rct linear map of vector spaces, presentation}
\StarST линейное отображение векторных пространств.
Пусть
\ShowEq{rcd vector space Basis f}
$\RCstar S$\Hyph  базис в векторном пространстве $\Vector V$
и
\ShowEq{rcd vector space Basis e}
$\RCstar T$\Hyph базис в векторном пространстве $\Vector U$.

Из определений
\ref{definition: rcs rct linear map of vector spaces} и
\ref{definition: morphism of representations of F algebra}
следует
\ShowEq{rcs rct linear map of vector spaces, presentation, 1}
\ShowEq{rcd linear map, 3i}
также вектор векторного пространства $\Vector U$ и имеет
разложение
\RcdMap{rcs rct linear map of vector spaces, presentation, 2}
относительно базиса $\Basis e$.
Комбинируя \EqRef{rcs rct linear map of vector spaces, presentation, 1}
и \EqRef{rcs rct linear map of vector spaces, presentation, 2}, мы получаем
\ShowEq{rcs rct linear map of vector spaces, presentation, 3}

Пусть $\Vector W$ - \rcd векторное пространство.
Пусть
\ShowEq{rct rcd linear map of vector spaces, presentation}
\StarTD линейное отображение векторных пространств.
Пусть
\ShowEq{rcd vector space Basis g}
\rcd  базис в векторном пространстве $\Vector W$.
Тогда, согласно
\EqRef{rcs rct linear map of vector spaces, presentation, 3},
произведение 
\StarST линейного отображения $(r,\Vector A)$ и
\StarTD линейного отображения $(p,\Vector B)$
имеет вид
\ShowEq{rcs rct linear map of vector spaces, presentation, 4}
Сопоставление равенств
\EqRef{product of rcd linear maps, C} и
\EqRef{rcs rct linear map of vector spaces, presentation, 4}
показывает насколько рассширеная теория линейных отображений
сложнее сокращённой теории.

При необходимости мы можем пользоваться рассширеной теорией,
но мы не получим новых результатов по сравнению со случаем
сокращённой теорией. В то же время обилие деталей
делает картину менее ясной и требует постоянного внимания.
\qed
\end{remark}

==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%A%0
\Symb%
   {$(^a_b)$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb%
   {минор}%
   {A from b a}%
\Symb%
   {минор}%
   {A from columns T}%
\Symb%
   {минор}%
   {A from rows S}%
\Symb%
   {минор}%
   {A without column a}%
\Symb%
   {минор}%
   {A without columns T}%
\Symb%
   {минор}%
   {A without row b}%
\Symb%
   {минор}%
   {A without rows S}%
\Symb%
   {аффинное пространство}%
   {affine space, division ring}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения $\Vector{A}$ $D$\Hyph векторного пространства}%
   {component of linear map, D vector space}%
\Symb%
   {компонента $p$ полиаддитивного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {лупа автоморфизмов представления $f$}%
   {loop of automorphisms of representation}%
\Symb%
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное аддитивное отображение переменной $v^i$}%
   {partial additive map of variable}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {множество аддитивных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set additive maps, D vector space}%
\Symb%
   {множество аддитивных отображений кольца $R_1$ в кольцо $R_2$}%
   {set additive maps, ring}%
\Symb%
   {множество полиаддитивных отображений}%
   {set polyadditive maps, D vector space}%
\Symb%
   {множество полиаддитивных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polyadditive maps, ring}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\mathcal{V}$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {многообразие \drc базисов аффинного пространства}%
   {drc Basis Manifold, Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {структурные константы алгебры $A$ над кольцом $R$}%
   {structural constants of algebra}%
\Symb%
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%

\SetIndexSpace%C%0
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {координаты базового вектора представления группы Ли}%
   {basis vector of representation of Lie group, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Symb%
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$ алгебры}%
   {Gateaux derivative of map, algebra}%
\Symb%
   {производная Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Symb%
   {производная Гато отображения $f$ алгебры}%
   {Gateaux derivative of map, fraction, algebra}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Symb%
   {производная Гато второго порядка отображения $\Vector f$}%
   {Gateaux derivative of Second Order, D vector space}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Symb%
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Symb%
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ тела}%
   {Gateaux differential of Second Order, division ring}%
\Symb%
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 1, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 2, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 3, D vector space}%
\Symb%
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Symb%
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 1, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 2, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 3, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {\drc векторное пространство \subs строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Symb%
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {аффинный базис}%
   {drc affine basis, division ring}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {активное представление лупы $\mathfrak A(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {координаты базиса в \rcd векторном пространстве \sups строк}%
   {basis coordinates, c rows rcd vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \subs строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \rcd векторного пространства \sups строк}%
   {basis, c rows rcd vector space}%
\Symb%
   {базис в \drc векторном пространстве \subs строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Symb%
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Symb%
   {норма отображения $f$  тела}%
   {norm of map, division ring}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормальный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная $F$\Hyph компонента аддитивного отображения $f$ }%
   {standard component of additive map, division ring}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная компонента линейного отображения $f$ тела}%
   {standard component of linear map, division ring}%
\Symb%
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро аддитивного отображения $D$\Hyph векторного пространства}%
   {kernel of additive map, D vector space}%
\Symb%
   {ядро аддитивного отображения тела}%
   {kernel of additive map, division ring}%

\SetIndexSpace%L%0
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Symb%
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {\rcd векторное пространство \drc линейных отображений \drc векторного пространства $\Vector V$ в \drc векторное пространство $\Vector W$}%
   {set drc linear maps, drc vector space}%
\Symb%
   {множество линейных отображений алгебры $A_1$ в алгебру $A_2$}%
   {set linear mappings, algebra}%
\Symb%
   {множество линейных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set linear maps, D vector space}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$  в модуль $S$}%
   {set polylinear mappings, algebra}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {\drc векторное пространство \rcd линейных отображений \rcd векторного пространства $\Vector{V}$ в \rcd векторное пространство $\Vector{W}$}%
   {set rcd linear maps, rcd vector space}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {\rcd векторное пространство \sups строк}%
   {c rows rcd vector space}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%
\Symb%
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%V%0
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J_f(X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {координаты пассивного отображения многообразия базисов представления}%
   {coordinates of passive map of basis manifold of representation}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%

\SetIndexSpace%X%0
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex


==> Tstar.Morphism.Russian.tex <==
%auto-ignore
\input{Tstar.Morphism}

\section{Представление универсальной алгебры}

\begin{definition}
Пусть на множестве $M$ определена структура $\Omega_2$\Hyph алгебры
(\citeBib{Burris Sankappanavar,Cohn: Universal Algebra}).
Мы будем называть эндоморфизм
$\Omega_2$\Hyph алгебры
\[
t:M\rightarrow M
\]
\AddIndex{преобразование универсальной алгебры}
{transformation of universal algebra} $M$.\footnote{Если множество
операций $\Omega_2$\Hyph алгебры пусто, то
$t$ является отображением.}
\qed
\end{definition}

Мы будем обозначать
\symb{\delta}1{identical transformation}
тождественное преобразование.

\begin{definition}
Преобразование называется
\AddIndex{левосторонним преобразованием}{left-side transformation}
или
\AddIndex{\Ts преобразованием}{Tstar transformation},
если оно действует слева
\[
u'=t u
\]
Мы будем обозначать
\symb{{}^\star M}1{set of Tstar transformations}
множество \Ts преобразований множества $M$.
\qed
\end{definition}

\begin{definition}
Преобразование называется
\AddIndex{правосторонним преобразованием}{right-side transformation}
или
\AddIndex{\sT преобразованием}{starT transformation},
если оно действует справа
\[
u'= ut
\]
Мы будем обозначать
\symb{M^\star}1{set of starT transformations}
множество \sT преобразований множества $M$.
\qed
\end{definition}

\begin{definition}
\label{definition: Tstar representation of algebra} 
Пусть на множестве ${}^\star M$ определена структура $\Omega_1$\Hyph алгебры
(\citeBib{Burris Sankappanavar}).
Пусть $A$ является $\Omega_1$\Hyph алгеброй.
Мы будем называть гомоморфизм
\begin{equation}
f:A\rightarrow {}^\star M
\label{eq: Tstar representation of algebra}
\end{equation}
\AddIndex{левосторонним}
{left-side representation of algebra} или
\AddIndex{\Ts представлением $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$}
{Tstar representation of algebra}
\qed
\end{definition}

\begin{definition}
\label{definition: starT representation of algebra} 
Пусть на множестве $M^\star$ определена структура $\Omega_1$\Hyph алгебры
(\citeBib{Burris Sankappanavar}).
Пусть $A$ является $\Omega_1$\Hyph алгеброй.
Мы будем называть гомоморфизм
\[
f:A\rightarrow M^\star
\]
\AddIndex{правосторонним}
{right-side representation of algebra} или
\AddIndex{\sT представлением $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$}
{starT representation of algebra}
\qed
\end{definition}

Мы распространим на теорию представлений соглашение,
описанное в замечании
\ePrints{0803.2620,0906.0135,0912.3315}
\ifx\Semafor\ValueOn
\xRef{0701.238}{remark: left and right matrix notation}.
\else
\ePrints{0501.237}
\ifx\Semafor\ValueOn
\xRef{0612.111}{remark: left and right matrix notation}.
\else
\ref{remark: left and right matrix notation}.
\fi
\fi
Мы можем записать принцип двойственности в следующей форме

\begin{theorem}[принцип двойственности]
\label{theorem: duality principle, algebra representation}
Любое утверждение, справедливое для
\Ts представления $\Omega_1$\Hyph алгебры $A$,
будет справедливо для \sT представления $\Omega_1$\Hyph алгебры $A$.
\end{theorem}

\begin{remark}
\label{remark: duality principle, algebra representation}
Существует две формы записи преобразования $\Omega_2$\Hyph алгебры $M$.
Если мы пользуемся операторной записью, то преобразование $A$
записывается в виде $Aa$ или $aA$, что соответствует
\Ts преобразованию или \sT преобразованию.
Если мы пользуемся функциональной записью, то преобразование $A$
записывается в виде $A(a)$ независимо от того, это
\Ts преобразование или \sT преобразование.
Эта запись согласована с принципом двойственности.

Это замечание является основой следующего соглашения.
Когда мы пользуемся функциональной записью, мы не различаем
\Ts преобразование и \sT преобразование.
Мы будем обозначать
\symb{{}^* M}1{set of transformations}
множество преобразований $\Omega_2$\Hyph алгебры $M$.
Пусть на множестве ${}^* M$ определена структура $\Omega_1$\Hyph алгебры.
Пусть $A$ является $\Omega_1$\Hyph алгеброй.
Мы будем называть гомоморфизм
\begin{equation}
f:A\rightarrow {}^* M
\label{eq: representation of algebra}
\end{equation}
\AddIndex{представлением $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$}
{representation of algebra}.

Соответствие между операторной записью и функциональной записью однозначно.
Мы можем выбирать любую форму записи, которая удобна для изложения конкретной темы.
\qed
\end{remark}

Диаграмма
\[
\xymatrix{
M\ar[rr]^{f(a)}&&M\\
&A\ar@{=>}[u]^f&
}
\]
означает, что мы рассматриваем представление $\Omega_1$\Hyph алгебры $A$.
Отображение $f(a)$ является образом $a\in A$.

\begin{definition}
\label{definition: effective representation of algebra}
Мы будем называть представление $\Omega_1$\Hyph алгебры $A$
\AddIndex{эффективным}{effective representation of algebra},
если отображение \EqRef{representation of algebra} -
изоморфизм $\Omega_1$\Hyph алгебры $A$ в ${}^* M$.
\qed
\end{definition}

\begin{remark}
\label{remark: notation for effective representation of algebra}
Если \Ts представление $\Omega_1$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\Omega_1$\Hyph алгебры с его образом и записывать \Ts преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=av\]
Если \sT представление $\Omega_1$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\Omega_1$\Hyph алгебры с его образом и записывать \sT преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=va\]
\qed
\end{remark}

\begin{definition}
\label{definition: transitive representation of algebra}
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и эффективно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\Ts представление однотранзитивно тогда и только тогда, когда для любых $a, b \in M$
существует одно и только одно $g\in A$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \ref{definition: effective representation of algebra}
и \ref{definition: transitive representation of algebra}.
\end{proof}

\section{Морфизм представлений
универсальной алгебры}

\begin{theorem}
Пусть $A$ и $B$ - $\Omega_1$\Hyph алгебры.
Представление $\Omega_1$\Hyph алгебры $B$
\[
g:B\rightarrow {}^\star M
\]
и гомоморфизм $\Omega_1$\Hyph алгебры
\begin{equation}
h:A\rightarrow B
\label{eq: homomorphism of algebra F}
\end{equation}
определяют представление $f$ $\Omega_1$\Hyph алгебры $A$
\[
\xymatrix{
A\ar[dr]^h\ar[rr]^f&&{}^* M\\
&B\ar[ur]^g&
}
\]
\end{theorem}
\begin{proof}
Отображение $f$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру ${}^* M$,
так как отображение $g$ является гомоморфизмом $\Omega_1$\Hyph алгебры $B$ в
$\Omega_1$\Hyph алгебру ${}^* M$.
\end{proof}

Если мы изучаем представление $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебрах $M$ и $N$, то нас интересуют отображения
из $M$ в $N$, сохраняющие структуру представления.

\begin{definition}
\label{definition: morphism of representations of F algebra}
Пусть
\[
f:A\rightarrow {}^* M
\]
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$ и 
\[
g:B\rightarrow {}^* N
\]
представление $\Omega_1$\Hyph алгебры $B$
в $\Omega_2$\Hyph алгебре $N$.
Пара отображений
\ShowEq{morphism of representations of F algebra, definition, 1}
таких, что
\begin{itemize}
\item $r$ - гомоморфизм $\Omega_1$\Hyph алгебры
\item $R$ - гомоморфизм $\Omega_2$\Hyph алгебры
\item
\begin{equation}
R\circ\textcolor{blue}{f(a)}=g(\textcolor{red}{r(a)})\circ R
\label{eq: morphism of representations of F algebra, definition, 2}
\end{equation}
\end{itemize}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
\qed
\end{definition}

Для произвольного $m\in M$ равенство
\EqRef{morphism of representations of F algebra, definition, 2}
имеет вид
\begin{equation}
\textcolor{blue}{R(f(a)(m))}=g(\textcolor{red}{r(a)})(\textcolor{blue}{R(m)})
\label{eq: morphism of representations of F algebra, definition, 2m}
\end{equation}

\begin{remark}
Мы можем рассматривать пару отображений $r$, $R$ как отображение
\[
F:A\cup M\rightarrow B\cup N
\] такое, что
\[
F(A)=B \ \ \ \ F(M)=N
\]
Поэтому в дальнейшем мы будем говорить, что дано отображение $(r,R)$.
\qed
\end{remark}

\begin{remark}
Рассмотрим морфизм представлений
\EqRef{morphism of representations of F algebra, definition, 1}.
Мы можем обозначать элементы множества $B$, пользуясь буквой по образцу $b\in B$.
Но если мы хотим показать, что $b$ является образом элемента $a\in A$,
мы будем пользоваться обозначением $\textcolor{red}{r(a)}$.
Таким образом, равенство
\[
\textcolor{red}{r(a)}=r(a)
\]
означает, что $\textcolor{red}{r(a)}$ (в левой части равенства)
является образом $a\in A$ (в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $N$ в виде $\textcolor{blue}{R(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами, где определены
соответствующие представления.

Мы можем интерпретировать
\EqRef{morphism of representations of F algebra, definition, 2m}
двумя способами
\begin{itemize}
\item Пусть преобразование $\textcolor{blue}{f(a)}$ отображает $m\in M$
в $\textcolor{blue}{f(a)}(m)$.
Тогда преобразование $g(\textcolor{red}{r(a)})$ отображает
$\textcolor{blue}{R(m)}\in N$ в $\textcolor{blue}{R(f(a)(m))}$.
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\[
\xymatrix{
&M\ar[dd]_(.3){f(a)}\ar[rr]^R&&N\ar[dd]^(.3){g(\textcolor{red}{r(a)})}\\
&\ar @{}[rr]|{(1)}&&\\
&M\ar[rr]^R&&N\\
A\ar[rr]^r\ar@{=>}[uur]^(.3)f&&B\ar@{=>}[uur]^(.3)g
}
\]
Из \EqRef{morphism of representations of F algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
\qed
\end{remark}

\begin{theorem}
\label{theorem: morphism of representations and algebra}
Рассмотрим представление
\[
f:A\rightarrow {}^* M
\]
$\Omega_1$\Hyph алгебры $A$ 
и представление
\[
g:B\rightarrow {}^* N
\]
$\Omega_1$\Hyph алгебры $B$.
Морфизм
\[
\xymatrix{
h:A\ar[r]&B&H:M\ar[r]&N
}
\]
представлений из $f$ в $g$
удовлетворяет соотношению
\begin{equation}
H\circ\omega(\textcolor{blue}{f(a_1)},...,\textcolor{blue}{f(a_n)})=
\omega(\textcolor{red}{g(h(a_1))},...,\textcolor{red}{g(h(a_n))})\circ H
\label{eq: morphism of representations of F algebra, 1}
\end{equation}
для произвольной $n$-арной операции $\omega$ $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Так как $f$ - гомоморфизм, мы имеем
\begin{equation}
H\circ\omega(\textcolor{blue}{f(a_1)},...,\textcolor{blue}{f(a_n)})
=H\circ\textcolor{blue}{f(\omega(a_1,...,a_n))}
\label{eq: morphism of representations of F algebra, 2}
\end{equation}
Из \EqRef{morphism of representations of F algebra, definition, 2} и
\EqRef{morphism of representations of F algebra, 2} следует
\begin{equation}
H\circ\omega(\textcolor{blue}{f(a_1)},...,\textcolor{blue}{f(a_n)})
=\textcolor{red}{g(h(\omega(a_1,...,a_n)))}\circ H
\label{eq: morphism of representations of F algebra, 3}
\end{equation}
Так как $h$ - гомоморфизм, из
\EqRef{morphism of representations of F algebra, 3} следует
\begin{equation}
H\circ\omega(\textcolor{blue}{f(a_1)},...,\textcolor{blue}{f(a_n)})
=\textcolor{red}{g(\omega(h(a_1),...,h(a_n)))}\circ H
\label{eq: morphism of representations of F algebra, 4}
\end{equation}
Так как $g$ - гомоморфизм, из
\EqRef{morphism of representations of F algebra, 4} следует
\EqRef{morphism of representations of F algebra, 1}.
\end{proof}

\begin{theorem}
\label{theorem: morphism of representations and homomorphism of algebra}
Пусть отображение
\[
\xymatrix{
h:A\ar[r]&B&H:M\ar[r]&N
}
\]
является морфизмом из представления
\[
f:A\rightarrow {}^* M
\]
$\Omega_1$\Hyph алгебры $A$ в представление
\[
g:B\rightarrow {}^* N
\]
$\Omega_1$\Hyph алгебры $B$.
Если представление $f$ эффективно, то отображение
\[
{}^*H:{}^* M\rightarrow{}^* N
\]
определённое равенством
\begin{equation}
{}^*H(\textcolor{blue}{f(a)})=\textcolor{red}{g(h(a))}
\label{eq: morphism of representations, star morphism}
\end{equation}
является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Так как представление $f$ эффективно, то для выбранного преобразования
$\textcolor{blue}{f(a)}$ выбор элемента $a$ определён однозначно.
Следовательно, преобразование $\textcolor{red}{g(h(a))}$
в равенстве \EqRef{morphism of representations, star morphism}
определено корректно.

Так как $f$ - гомоморфизм, мы имеем
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))={}^*H(f(\omega(a_1,...,a_n)))
\label{eq: morphism of representations, star morphism, 2}
\end{equation}
Из \EqRef{morphism of representations, star morphism} и
\EqRef{morphism of representations, star morphism, 2} следует
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))=g(h(\omega(a_1,...,a_n)))
\label{eq: morphism of representations, star morphism, 3}
\end{equation}
Так как $h$ - гомоморфизм, из
\EqRef{morphism of representations, star morphism, 3} следует
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))=g(\omega(h(a_1),...,h(a_n)))
\label{eq: morphism of representations, star morphism, 4}
\end{equation}
Так как $g$ - гомоморфизм,
\[
{}^*H(\omega(f(a_1),...,f(a_n)))=\omega(g(h(a_1)),...,g(h(a_n)))
=\omega({}^*H(f(a_1)),...,{}^*H(f(a_n)))
\]
следует из \EqRef{morphism of representations, star morphism, 4}.
Следовательно, отображение ${}^*H$ является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{proof}

\begin{theorem}
\label{theorem: morphism of representations of F algebra}
Если представление
\[
f:A\rightarrow {}^* M
\]
$\Omega_1$\Hyph алгебры $A$ однотранзитивно и представление
\[
g:B\rightarrow {}^* N
\]
$\Omega_1$\Hyph алгебры $B$ однотранзитивно,
то существует морфизм
\[
\xymatrix{
h:A\ar[r]&B&H:M\ar[r]&N
}
\]
представлений из $f$ в $g$.
\end{theorem}
\begin{proof}
Выберем гомоморфизм $h$.
Выберем элемент $m\in M$
и элемент $n\in N$. 
Чтобы построить отображение $H$, рассмотрим следующую диаграмму
\[
\xymatrix{
&M\ar[dd]^(.3)a\ar[rr]^H&&N\ar[dd]_(.3){h(a)}\\
&\ar @{}[rr]|{(1)}&&\\
&M\ar[rr]^H&&N\\
A\ar[rr]^h\ar@{=>}[uur]^(.3)f&&B\ar@{=>}[uur]^(.3)g
}
\]
Из коммутативности диаграммы $(1)$ следует
\[
H(am)=h(a)H(m)
\]
Для произвольного $m'\in M$ однозначно определён $a\in A$ такой,
что $m'=am$. Следовательно, мы построили отображении $H$,
которое удовлетворяет равенству
\EqRef{morphism of representations of F algebra, definition, 2}.
\end{proof}

\begin{theorem}
\label{theorem: uniq morphism of representations of F algebra}
Если представление
\[
f:A\rightarrow {}^* M
\]
$\Omega_1$\Hyph алгебры $A$ однотранзитивно и представление
\[
g:B\rightarrow {}^* N
\]
$\Omega_1$\Hyph алгебры $B$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\[
\xymatrix{
h:A\ar[r]&B
}
\]
отображение
\[
\xymatrix{
H:M\ar[r]&N
}
\]
такое, что $(h,H)$ является морфизмом
представлений из $f$ в $g$,
единственно
с точностью до выбора образа $n=H(m)\in N$
заданного элемента $m\in M$.
\end{theorem}
\begin{proof}
Из доказательства теоремы
\ref{theorem: morphism of representations of F algebra}
следует, что выбор гомоморфизма $h$ и элементов
$m\in M$, $n\in N$ однозначно определяет отображение $H$.
\end{proof}

\begin{theorem}
Если представление
\[
f:A\rightarrow {}^* M
\]
$\Omega_1$\Hyph алгебры $A$ однотранзитивно,
то для любого эндоморфизма $\Omega_1$\Hyph алгебры $A$ существует эндоморфизм
\[
\xymatrix{
p:A\ar[r]&A&P:M\ar[r]&M
}
\]
представления $f$.
\end{theorem}
\begin{proof}
Рассмотрим следующую диаграмму
\[
\xymatrix{
&M\ar[dd]^(.3)a\ar[rr]^H&&M\ar[dd]_(.3){p(a)}\\
&\ar @{}[rr]|{(1)}&&\\
&M\ar[rr]^H&&M\\
A\ar[rr]^p\ar@{=>}[uur]^(.3)f&&A\ar@{=>}[uur]^(.3)f
}
\]
Утверждение теоремы является следствием теоремы
\ref{theorem: morphism of representations of F algebra}.
\end{proof}

\begin{theorem}
\label{theorem: product of morphisms of representations of F algebra}
Пусть
\[
f:A\rightarrow {}^* M
\]
представление $\Omega_1$\Hyph алгебры $A$,
\[
g:B\rightarrow {}^* N
\]
представление $\Omega_1$\Hyph алгебры $B$,
\[
h:C\rightarrow {}^* L
\]
представление $\Omega_1$\Hyph алгебры $C$.
Пусть определены морфизмы представлений $\Omega_1$\Hyph алгебры
\[
\xymatrix{
p:A\ar[r]&B&P:M\ar[r]&N
}
\]
\[
\xymatrix{
q:B\ar[r]&C&Q:N\ar[r]&L
}
\]
Тогда определён морфизм представлений $\Omega_1$\Hyph алгебры
\[
\xymatrix{
r:A\ar[r]&C&R:M\ar[r]&L
}
\]
где $r=qp$, $R=QP$.
Мы будем называть морфизм $(r,R)$ представлений из $f$ в $h$
\AddIndex{произведением морфизмов $(p,P)$ и $(q,Q)$
представлений универсальной алгебры}
{product of morphisms of representations of universal algebra}.
\end{theorem}
\begin{proof}
Мы можем представить утверждение теоремы,
пользуясь диаграммой
\[
\xymatrix{
&&N\ar[rrrrr]^Q&&&
&&L
\\
&&&&&&&
\\
B\ar[r]^q\ar@/^2pc/@{=>}[urrr]^g&
C\ar@{=>}[urrrrr]^(.4)h&&&
N\ar[r]^Q\ar[lluu]_{g(\textcolor{red}{p(a)})}&
L\ar[rruu]_(.3){h(\textcolor{red}{r(a)})}
\\
A\ar[u]^p\ar@/_2pc/[ur]_r\ar@/_2pc/@{=>}[drrr]^f
&&&&
M\ar[u]^P\ar[ddll]^(.3){f(a)}\ar@/_1pc/[ru]_R
\\
&&&&&&&
\\
&&M\ar[uuuuu]^P\ar@/_5pc/[rrrrruuuuu]_R
}
\]
Отображение $r$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру $C$.
Нам надо показать, что пара отображений $(r,R)$ удовлетворяет
\EqRef{morphism of representations of F algebra, definition, 2}:
\begin{align*}
\textcolor{blue}{R(f(a)m)}&=\textcolor{blue}{QP(f(a)m)}\\
&=\textcolor{blue}{Q(g(\textcolor{red}{p(a)})\textcolor{blue}{P(m)})}\\
&=h(\textcolor{red}{qp(a)})\textcolor{blue}{QP(m)})\\
&=h(\textcolor{red}{r(a)})\textcolor{blue}{R(m)}
\end{align*}
\end{proof}

\begin{definition}
\label{definition: category of representations of F algebra from category}
Допустим $\mathcal A$ категория $\Omega_1$\Hyph алгебр.
Мы определим \AddIndex{категорию
\symb{T\star\mathcal A}1
{category of Tstar representations of Omega1 algebra from category}
$\ $ \Ts представлений универсальной алгебры
из категории $\mathcal A$}
{category of Tstar representations of Omega1 algebra from category}.
Объектами этой категории являются \Ts представлениями $\Omega_1$\Hyph алгебры.
Морфизмами этой категории являются морфизмы \Ts представлений $\Omega_1$\Hyph алгебры.
\qed
\end{definition}

\begin{theorem}
Эндоморфизмы представления $f$ порождают полугруппу.
\end{theorem}
\begin{proof}
Из теоремы
\ref{theorem: product of morphisms of representations of F algebra}
следует, что произведение эндоморфизмов $(p,P)$, $(r,R)$ представления $f$
является эндоморфизмом $(pr,PR)$ представления $f$.
\end{proof}

\begin{definition}
Пусть на множестве $M$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия $m_1\equiv m_2(\mathrm{mod} S)$ следует
$f(m_1)\equiv f(m_2)(\mathrm{mod} S)$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: transformation correlated with equivalence}
Пусть на множестве $M$ определена эквивалентность $S$.
Пусть на множестве ${}^* M$ определена $\Omega_1$\Hyph алгебра.
Если преобразования согласованны с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве ${}^*(M/S)$.
\end{theorem}
\begin{proof}
Пусть $h=\mathrm{nat}\ S$. Если $m_1\equiv m_2(\mathrm{mod} S)$,
то $h(m_1)=h(m_2)$. Поскольку
$f\in{}^* M$ согласованно с эквивалентностью $S$,
то $h(f(m_1))=h(f(m_2))$. Это позволяет определить
преобразование $F$ согласно правилу
\[
F([m])=h(f(m))
\]

Пусть $\omega$ - n\Hyph арная операция $\Omega_1$\Hyph алгебры.
Пусть $f_1$, ..., $f_n\in{}^\star M$ и
\ShowEq{morphism of representations and equivalence}
Мы определим операцию на множестве ${}^\star(M/S)$ по правилу
\[
\omega(F_1,...,F_n)[m]=h(\omega(f_1,...,f_n)m)
\]
Это определение корректно, так как
$\omega(f_1,...,f_n)\in{}^\star M$ и согласованно с эквивалентностью $S$.
\end{proof}

\begin{theorem}
\label{theorem: decompositions of morphism of representations}
Пусть
\[
f:A\rightarrow {}^* M
\]
представление $\Omega_1$\Hyph алгебры $A$,
\[
g:B\rightarrow {}^* N
\]
представление $\Omega_1$\Hyph алгебры $B$.
Пусть
\[
\xymatrix{
r:A\ar[r]&B&R:M\ar[r]&N
}
\]
морфизм представлений из $f$ в $g$.
Положим
\begin{align*}
s&=rr^{-1}&S&=RR^{-1}
\end{align*}
Тогда для отображений $r$, $R$ существуют разложения,
которые можно описать диаграммой
\[
\xymatrix{
&&M/S\ar[rrrrr]^T\ar@{}[drrrrr]|{(5)}&&\ar@{}[dddddll]|{(4)}&
\ar@{}[dddddrr]|{(6)}&&RM\ar[ddddd]^I\\
&&&&&&&\\
A/s\ar[r]^t\ar@/^2pc/@{=>}[urrr]^F&
rA\ar[d]^i\ar@{=>}[urrrrr]^(.4)G&&&
M/S\ar[r]^T\ar[lluu]_{F(\textcolor{red}{j(a)})}&
RM\ar[d]^I\ar[rruu]_{G(\textcolor{red}{r(a)})}\\
A\ar[r]_r\ar[u]^j\ar@{}[ur]|{(1)}\ar@/_2pc/@{=>}[drrr]^f&
B\ar@{=>}[drrrrr]^(.4)g&&&
M\ar[r]_R\ar[u]^J\ar@{}[ur]|{(2)}\ar[ddll]^{f(a)}&
N\ar[ddrr]^{g(\textcolor{red}{r(a)})}\\
&&&&&&&\\
&&M\ar[uuuuu]^J\ar[rrrrr]_R\ar@{}[urrrrr]|{(3)}&&&&&N
}
\]
\begin{enumerate}
\item $s=\mathrm{ker}\ r$ является конгруэнцией на $A$.
Существует разложение гомоморфизма $r$
\begin{equation}
r=itj
\label{eq: morphism of representations of algebra, homomorphism, 1}
\end{equation}
$j=\mathrm{nat}\ s$ - естественный гомоморфизм
\begin{equation}
\textcolor{red}{j(a)}=j(a)
\label{eq: morphism of representations of algebra, homomorphism, 2}
\end{equation}
$t$ - изоморфизм
\begin{equation}
\textcolor{red}{r(a)}=t(\textcolor{red}{j(a)})
\label{eq: morphism of representations of algebra, homomorphism, 3}
\end{equation}
$i$ - вложение
\begin{equation}
r(a)=i(\textcolor{red}{r(a)})
\label{eq: morphism of representations of algebra, homomorphism, 4}
\end{equation}
\item $S=\mathrm{ker}\ R$ является эквивалентностью на $M$.
Существует разложение отображения $R$
\begin{equation}
R=ITJ
\label{eq: morphism of representations of algebra, map, 1}
\end{equation}
$J=\mathrm{nat}\ S$ - сюръекция
\begin{equation}
\textcolor{blue}{J(m)}=J(m)
\label{eq: morphism of representations of algebra, map, 2}
\end{equation}
$T$ - биекция
\begin{equation}
\textcolor{blue}{R(m)}=T(\textcolor{blue}{J(m)})
\label{eq: morphism of representations of algebra, map, 3}
\end{equation}
$I$ - вложение
\begin{equation}
R(m)=I(\textcolor{blue}{R(m)})
\label{eq: morphism of representations of algebra, map, 4}
\end{equation}
\item $F$ - \Ts представление $\Omega_1$\Hyph алгебры $A/s$ в $M/S$
\item $G$ - \Ts представление $\Omega_1$\Hyph алгебры $rA$ в $RM$
\item $(j,J)$ - морфизм представлений $f$ и $F$
\label{theorem: (j,J) is morphism of representations}
\item $(t,T)$ - морфизм представлений $F$ и $G$
\label{theorem: (t,T) is morphism of representations}
\item $(t^{-1},T^{-1})$ - морфизм представлений $G$ и $F$
\label{theorem: (t-1,T-1) is morphism of representations}
\item $(i,I)$ - морфизм представлений $G$ и $g$
\label{theorem: (i,I) is morphism of representations}
\item Существует разложение морфизма представлений
\ShowEq{decompositions of morphism of representations}
\label{theorem: exists decompositions of morphism of representations}
\end{enumerate} 
\end{theorem}
\begin{proof}
Существование диаграмм $(1)$ и $(2)$ следует из теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, с. 74).
%Существование диаграммы $(2)$ следует из теоремы I.3.1
%(\citeBib{Cohn: Universal Algebra}, с. 28).

Мы начнём с диаграммы $(4)$.

Пусть $m_1\equiv m_2(\mathrm{mod}\ S)$.
%Тогда $J(m_1)=J(m_2)$,
Следовательно,
\begin{equation}
\textcolor{blue}{R(m_1)}=\textcolor{blue}{R(m_2)}
\label{eq: morphism of representations of algebra, (4), 1}
\end{equation}
%$JT(m_1)=JT(m_2)$,
%так как $JT$ - отображение на $MR$.
Если $a_1\equiv a_2(\mathrm{mod}s)$, то
\begin{equation}
\textcolor{red}{r(a_1)}=\textcolor{red}{r(a_2)}
\label{eq: morphism of representations of algebra, (4), 2}
\end{equation}
Следовательно,
$j(a_1)=j(a_2)$.
Так как $(r,R)$ - морфизм представлений, то
\begin{equation}
\textcolor{blue}{R(f(a_1)(m_1))}=g(\textcolor{red}{r(a_1)})(\textcolor{blue}{R(m_1)})
\label{eq: morphism of representations of algebra, (4), 3}
\end{equation}
\begin{equation}
\textcolor{blue}{R(f(a_2)(m_2))}=g(\textcolor{red}{r(a_2)})(\textcolor{blue}{R(m_2)})
\label{eq: morphism of representations of algebra, (4), 4}
\end{equation}
Из \EqRef{morphism of representations of algebra, (4), 1},
\EqRef{morphism of representations of algebra, (4), 2},
\EqRef{morphism of representations of algebra, (4), 3},
\EqRef{morphism of representations of algebra, (4), 4}
следует
\begin{equation}
\textcolor{blue}{R(f(a_1)(m_1))}=\textcolor{blue}{R(f(a_2)(m_2))}
\label{eq: morphism of representations of algebra, (4), 5}
\end{equation}
Из \EqRef{morphism of representations of algebra, (4), 5}
следует
\begin{equation}
f(a_1)(m_1)\equiv f(a_2)(m_2)(\mathrm{mod} S)
\label{eq: morphism of representations of algebra, (4), 6}
\end{equation}
и, следовательно,
\begin{equation}
\textcolor{blue}{J(f(a_1)(m_1))}=\textcolor{blue}{J(f(a_2)(m_2))}
\label{eq: morphism of representations of algebra, (4), 7}
\end{equation}
Из \EqRef{morphism of representations of algebra, (4), 7}
следует, что отображение
\begin{equation}
F(\textcolor{red}{j(a)})(\textcolor{blue}{J(m)})
=\textcolor{blue}{J(f(a)(m)))}
\label{eq: morphism of representations of algebra, (4), 8}
\end{equation}
определено корректно и является преобразованием множества $M/S$.

Из равенства
\EqRef{morphism of representations of algebra, (4), 6}
(в случае $a_1=a_2$) следует, что для любого $a$ преобразование
согласованно с эквивалентностью $S$.
Из теоремы
\ref{theorem: transformation correlated with equivalence} следует,
что на множестве ${}^*(M/S)$ определена структура $\Omega_1$\Hyph алгебры.
Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
преобразований
\ShowEq{transformation correlated with equivalence, 1}
пространства $M/S$. Мы положим
\[
\omega(F(\textcolor{red}{j(a_1)}),...,F(\textcolor{red}{j(a_n)}))
(\textcolor{blue}{J(m)})=
J(\omega(f(a_1),...,f(a_n)))(m))
\]
Следовательно, отображение $F$ является представлением
$\Omega_1$\Hyph алгебры $A/s$.

Из \EqRef{morphism of representations of algebra, (4), 8}
следует, что $(j,J)$ является морфизмом представлений $f$ и $F$
(утверждение \eqref{theorem: (j,J) is morphism of representations}
теоремы).

Рассмотрим диаграмму $(5)$.

Так как $T$ - биекция, то мы можем отождествить элементы множества
$M/S$ и множества $MR$, причём это отождествление имеет вид
\begin{equation}
T(\textcolor{blue}{J(m)})=\textcolor{blue}{R(m)}
\label{eq: morphism of representations of algebra, (5), 1}
\end{equation}
Мы можем записать преобразование $F(\textcolor{red}{j(a)})$
множества $M/S$ в виде
\begin{equation}
F(\textcolor{red}{j(a)}):\textcolor{blue}{J(m)}\rightarrow
F(\textcolor{red}{j(a)})(\textcolor{blue}{J(m)})
\label{eq: morphism of representations of algebra, (5), 2}
\end{equation}
Так как $T$ - биекция, то мы можем определить преобразование
\begin{equation}
T(\textcolor{blue}{J(m)})\rightarrow
T(F(\textcolor{red}{j(a)})(\textcolor{blue}{J(m)}))
\label{eq: morphism of representations of algebra, (5), 3}
\end{equation}
множества $RM$. Преобразование
\EqRef{morphism of representations of algebra, (5), 3}
зависит от $\textcolor{red}{j(a)}\in A/s$.
Так как $t$ - биекция, то мы можем отождествить элементы множества
$A/s$ и множества $rA$, причём это отождествление имеет вид
\ShowEq{morphism of representations of algebra, (5), 6}
Следовательно, мы определили отображение
\[
G:rA\rightarrow{}^\star RM
\]
согласно равенству
\begin{equation}
G(t(\textcolor{red}{j(a)}))(T(\textcolor{blue}{J(m)}))=
T(F(\textcolor{red}{j(a)})(\textcolor{blue}{J(m)}))
\label{eq: morphism of representations of algebra, (5), 4}
\end{equation}

Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
преобразований
\ShowEq{morphism of representations of algebra, (5), 7}
пространства $RM$. Мы положим
\ShowEq{morphism of representations of algebra, (5), 5}
Согласно \EqRef{morphism of representations of algebra, (5), 4}
операция $\omega$ корректно определена на множестве ${}^\star RM$.
Следовательно, отображение $G$ является представлением
$\Omega_1$\Hyph алгебры.

Из \EqRef{morphism of representations of algebra, (5), 4}
следует, что $(t,T)$ является морфизмом представлений $F$ и $G$
(утверждение \eqref{theorem: (t,T) is morphism of representations}
теоремы).

Так как $T$ - биекция, то из равенства
\EqRef{morphism of representations of algebra, (5), 1}
следует
\begin{equation}
\textcolor{blue}{J(m)}=T^{-1}(\textcolor{blue}{R(m)})
\label{eq: morphism of representations of algebra, (5), 1a}
\end{equation}
Мы можем записать преобразование $G(\textcolor{red}{r(a)})$
множества $RM$ в виде
\ShowEq{morphism of representations of algebra, (5), 2a}
Так как $T$ - биекция, то мы можем определить преобразование
\ShowEq{morphism of representations of algebra, (5), 3a}
множества $M/S$. Преобразование
\EqRef{morphism of representations of algebra, (5), 3a}
зависит от $\textcolor{red}{r(a)}\in rA$.
Так как $t$ - биекция, то из равенства
\EqRef{morphism of representations of algebra, (5), 6}
следует
\ShowEq{morphism of representations of algebra, (5), 6a}
Так как по построению диаграмма $(5)$ коммутативна, то преобразование
\EqRef{morphism of representations of algebra, (5), 3a}
совпадает с преобразованием
\EqRef{morphism of representations of algebra, (5), 2}.
Равенство
\EqRef{morphism of representations of algebra, (5), 5}
можно записать в виде
\ShowEq{morphism of representations of algebra, (5), 5a}
Следовательно, $(t^{-1},T^{-1})$ является морфизмом представлений $G$ и $F$
(утверждение \eqref{theorem: (t-1,T-1) is morphism of representations}
теоремы).

Диаграмма $(6)$ является самым простым случаем в нашем доказательстве.
Поскольку отображение $I$ является вложением и диаграмма $(2)$
коммутативна, мы можем отождествить $n\in N$ и $\textcolor{blue}{R(m)}$,
если $n\in\textrm{Im}R$. Аналогично, мы можем отождествить
соответствующие преобразования.
\begin{equation}
g'(i(\textcolor{red}{r(a)}))(I(\textcolor{blue}{R(m)}))=
I(G(\textcolor{red}{r(a)})(\textcolor{blue}{R(m)}))
\label{eq: morphism of representations of algebra, (6), 1}
\end{equation}
\[
\omega(g'(\textcolor{red}{r(a_1)}),...,g'(\textcolor{red}{r(a_n)}))
(\textcolor{blue}{R(m)})=
I(\omega(G(\textcolor{red}{r(a_1)},...,G(\textcolor{red}{r(a_n)}))
(\textcolor{blue}{R(m)}))
\]
Следовательно,
$(i,I)$ является морфизмом представлений $G$ и $g$
(утверждение \eqref{theorem: (i,I) is morphism of representations}
теоремы).

Для доказательства утверждения
\eqref{theorem: exists decompositions of morphism of representations}
теоремы осталось показать, что определённое
в процессе доказательства представление $g'$ совпадает
с представлением $g$, а операции над преобразованиями совпадают
с соответствующими операциями на ${}^* N$.
\begin{align*}
g'(i(\textcolor{red}{r(a)}))(I(\textcolor{blue}{R(m)}))
&=I(G(\textcolor{red}{r(a)})(\textcolor{blue}{R(m)}))
&&\textrm{согласно}\ \EqRef{morphism of representations of algebra, (6), 1}\\
&=I(G(t(\textcolor{red}{j(a)}))(T(\textcolor{blue}{J(m)})))
&&\textrm{согласно}\ \EqRef{morphism of representations of algebra, homomorphism, 3},
\EqRef{morphism of representations of algebra, map, 3}\\
&=IT(F(\textcolor{red}{j(a)})(\textcolor{blue}{J(m)}))
&&\textrm{согласно}\ \EqRef{morphism of representations of algebra, (5), 4}\\
&=ITJ(f(a)(m))
&&\textrm{согласно}\ \EqRef{morphism of representations of algebra, (4), 8}\\
&=R(f(a)(m))
&&\textrm{согласно}\ \EqRef{morphism of representations of algebra, map, 1}\\
&=g(r(a))(R(m))
&&\textrm{согласно}\ \EqRef{morphism of representations of F algebra, definition, 2}
\end{align*}
\begin{align*}
\omega(G(\textcolor{red}{r(a_1)}),...,G(\textcolor{red}{r(a_n)}))
(\textcolor{blue}{R(m)})
&=T(\omega(F(\textcolor{red}{j(a_1)},...,F(\textcolor{red}{j(a_n)}))
(\textcolor{blue}{J(m)}))\\
&=T(F(\omega(\textcolor{red}{j(a_1)},...,\textcolor{red}{j(a_n)}))
(\textcolor{blue}{J(m)}))\\
&=T(F(j(\omega(a_1,...,a_n)))
(\textcolor{blue}{J(m)}))\\
&=T(J(f(\omega(a_1,...,a_n))(m)))\\
\end{align*}
\end{proof}

\begin{definition}
\label{definition: isomorphism of repesentations of Omega algebra}
Пусть
\[
f:A\rightarrow {}^* M
\]
представление $\Omega_1$\Hyph алгебры $A$,
\[
g:B\rightarrow {}^* N
\]
представление $\Omega_1$\Hyph алгебры $B$.
Пусть
\[
\xymatrix{
r:A\ar[r]&B&R:M\ar[r]&N
}
\]
морфизм представлений из $r$ в $R$ такой, что
$f$ - изоморфизм $\Omega_1$\Hyph алгебры и $g$
- изоморфизм $\Omega_2$\Hyph алгебры.
Тогда отображение $(r,R)$ называется
\AddIndex{изоморфизмом представлений}
{isomorphism of repesentations of Omega algebra}.
\qed
\end{definition}

\begin{theorem}
В разложении \EqRef{decompositions of morphism of representations}
отображение $(t,T)$ является изоморфизмом представлений $F$ и $G$.
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: isomorphism of repesentations of Omega algebra}
и утверждений \eqref{theorem: (t,T) is morphism of representations}
и \eqref{theorem: (t-1,T-1) is morphism of representations}
теоремы \ref{theorem: decompositions of morphism of representations}.
\end{proof}

Из теоремы \ref{theorem: decompositions of morphism of representations}
следует, что мы можем свести задачу изучения морфизма представлений
$\Omega_1$\Hyph алгебры
к случаю, описываемому диаграммой
\begin{equation}
\xymatrix{
&M\ar[dd]_(.3){f(a)}\ar[rr]^J&&M/S\ar[dd]^(.3){F(\textcolor{red}{j(a)})}\\
&&&\\
&M\ar[rr]^J&&M/S\\
A\ar[rr]^j\ar@{=>}[uur]^(.3)f&&A/s\ar@{=>}[uur]^(.3)F
}
\label{eq: morphism of representations of algebra, reduce, 1}
\end{equation}

\begin{theorem}
\label{theorem: morphism of representations of algebra, reduce}
Диаграмма \EqRef{morphism of representations of algebra, reduce, 1}
может быть дополнена представлением $F_1$
$\Omega_1$\Hyph алгебры $A$ в множестве $M/S$ так,
что диаграмма
\begin{equation}
\xymatrix{
&M\ar[dd]_(.3){f(a)}\ar[rr]^J&&M/S\ar[dd]^(.3){F(\textcolor{red}{j(a)})}\\
&&&\\
&M\ar[rr]^(.65)J&&M/S\\
A\ar[rr]^j\ar@{=>}[uur]^(.3)f\ar@{=>}[uurrr]^(.7){F_1}&&A/s\ar@{=>}[uur]^(.3)F
}
\label{eq: morphism of representations of algebra, reduce, 2}
\end{equation}
коммутативна. При этом множество преобразований представления $F$ и
множество преобразований представления $F_1$ совпадают.
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно положить
\[F_1(a)=F(\textcolor{red}{j(a)})\]
Так как отображение $j$ - сюрьекция, то $\mathrm{Im}F_1=\mathrm{Im}F$.
Так как $j$ и $F$ - гомоморфизмы $\Omega_1$\Hyph алгебры, то $F_1$
- также гомоморфизм $\Omega_1$\Hyph алгебры.
\end{proof}

Теорема \ref{theorem: morphism of representations of algebra, reduce}
завершает цикл теорем, посвящённых структуре морфизма представлений
$\Omega_1$\Hyph алгебры.
Из этих теорем следует, что мы можем упростить задачу изучения морфизма представлений
$\Omega_1$\Hyph алгебры и ограничиться морфизмом представлений вида
\[
\xymatrix{
id:A\ar[r]&A&R:M\ar[r]&N
}
\]
В этом случае мы можем отождествить морфизм $(id,R)$ представлений
$\Omega_1$\Hyph алгебры и отображение $R$.
Мы будем пользоваться диаграммой
\[
\xymatrix{
&M\ar[dd]_(.3){f(a)}\ar[rr]^R&&N\ar[dd]^(.3){g(a)}\\
&&&\\
&M\ar[rr]^(.65)R&&N\\
A\ar@{=>}[uur]^(.3)f\ar@{=>}[uurrr]^(.7)g
}
\]
для представления морфизма $(id,R)$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of F algebra}

Мы дадим следующее определение по аналогии с определением
\ref{definition: category of representations of F algebra from category}.

\begin{definition}
\label{definition: category of Tstar representations of Omega1 algebra}
Мы определим \AddIndex{категорию
\symb{T\star A}1{category of Tstar representations of Omega1 algebra}
$\ $ \Ts представлений $\Omega_1$\Hyph алгебры $A$}
{category of Tstar representations of Omega1 algebra}.
Объектами этой категории являются \Ts представлениями $\Omega_1$\Hyph алгебры $A$.
Морфизмами этой категории являются морфизмы $(id,R)$ \Ts представлений $\Omega_1$\Hyph алгебры $A$.
\qed
\end{definition}

\section{Автоморфизм представления
универсальной алгебры}

\begin{definition}
\label{definition: endomorphism of representation of F algebra}
Пусть
\[
f:A\rightarrow {}^* M
\]
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{morphism of representation of A in M}
такой, что $r$ - эндоморфизм $\Omega_1$\Hyph алгебры и
$R$ - эндоморфизм $\Omega_2$\Hyph алгебры
называется
\AddIndex{эндоморфизмом представления}
{endomorphism of representation} $f$.
\qed
\end{definition}

\begin{definition}
\label{definition: automorphism of representation of F algebra}
Пусть
\ShowEq{representation of F algebra}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{morphism of representation of A in M}
такой, что $r$ - автоморфизм $\Omega_1$\Hyph алгебры и
$R$ - автоморфизм $\Omega_2$\Hyph алгебры
называется
\AddIndex{автоморфизмом представления}
{automorphism of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: loop of automorphisms of representation}
Пусть
\ShowEq{representation of F algebra}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Множество автоморфизмов представления $f$
порождает \AddIndex{лупу}{loop of automorphisms of representation}
\ShowEq{loop of automorphisms of representation}.\footnote{Определение
лупы приведенно в
\citeBib{Sabinin: Smooth Quasigroups}, с. 24,
\citeBib{Kurosh: General Algebra}, с. 39.}
\end{theorem}
\begin{proof}
Пусть $(r,R)$, $(p,P)$ - автоморфизмы представления $f$.
Согласно определению
\ref{definition: automorphism of representation of F algebra}
отображения $r$, $p$ являются автоморфизмами
$\Omega_1$\Hyph алгебры $A$ и отображения $R$, $P$
являются автоморфизмами
$\Omega_2$\Hyph алгебры $M$.
Согласно теореме II.3.2
(\citeBib{Cohn: Universal Algebra}, c. 60)
отображение $rp$ является автоморфизмом
$\Omega_1$\Hyph алгебры $A$ и отображение $RP$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Из теоремы
\ref{theorem: product of morphisms of representations of F algebra}
и определения
\ref{definition: automorphism of representation of F algebra}
следует, что произведение автоморфизмов
$(rp,RP)$ представления $f$ является автоморфизмом представления $f$.

Пусть $(r,R)$ - автоморфизм представления $f$.
Согласно определению
\ref{definition: automorphism of representation of F algebra}
отображение $r$ является автоморфизмом
$\Omega_1$\Hyph алгебры $A$ и отображение $R$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Следовательно, отображение $r^{-1}$ является автоморфизмом
$\Omega_1$\Hyph алгебры $A$ и отображение $R^{-1}$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Для автоморфизма $(r,R)$ справедливо равенство
\EqRef{morphism of representations of F algebra, definition, 2m}.
Положим $a'=r(a)$, $m'=R(m)$. Так как $r$ и $R$ - автоморфизмы,
то $a=r^{-1}(a')$, $m=R^{-1}(m')$
и равенство
\EqRef{morphism of representations of F algebra, definition, 2m}
можно записать в виде
\ShowEq{morphism of representations of F algebra, definition, 2m-1}аа
Так как отображение $R$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$,
то из равенства
\EqRef{morphism of representations of F algebra, definition, 2m-1}
следует
\ShowEq{morphism of representations of F algebra, definition, 2m-1, 1}
Равенство
\EqRef{morphism of representations of F algebra, definition, 2m-1, 1}
соответствует равенству
\EqRef{morphism of representations of F algebra, definition, 2m}
для отображения $(r^{-1},R^{-1})$.
Следовательно, отображение $(r^{-1},R^{-1})$ является автоморфизмом
представления $f$.
\end{proof}

\begin{remark}
Очевидно, что множество автоморфизмов $\Omega_1$\Hyph алгебры $A$
также порождает лупу. Конечно,
заманчиво предположить, что множество автоморфизмов порождает
группу. Так как произведение автоморфизмов $f$ и $g$ является
автоморфизмом $fg$, то определены автоморфизмы $(fg)h$ и $f(gh)$.
Но из этого утверждения не следует, что
\[
(fg)h=f(gh)
\]
\qed
\end{remark}


==> Vector.Space.Russian.tex <==
%auto-ignore
\input{Vector.Space}
\ifx\PrintBook\Defined
\chapter{Векторное пространство над телом}
\label{chapter: Vector Space Over Division Ring}
\fi

\section{Векторное пространство}
\label{section: Vector Space}

Чтобы определить \Ts представление
\[
f:R\rightarrow {}^\star \Vector{M}
\]
кольца $R$ на множестве $\Vector{M}$
мы должны определить структуру кольца на множестве ${}^\star \Vector{M}$.\footnote{Можно
ли определить операцию сложения на множестве
${}^\star \Vector{M}$, если эта операция не определена на множестве
$\Vector{M}$. Ответ на этот вопрос положительный.

Допустим $\Vector{M}=B\cup C$ и $F:B\rightarrow C$ - взаимно однозначное
отображение. Мы определим множество ${}^\star \Vector{M}$ \Ts преобразований
множества $\Vector{M}$ согласно следующему правилу. Пусть $V\subseteq B$. \Ts отображение
$F_V$ имеет вид
\[
F_Vx=\left\{\begin{array}{lr}
x&x\in B\backslash V\\
Fx&x\in V  \\
x&x\in C\backslash F(V)\\
F^{-1}x&x\in F(V)  
\end{array}\right.
\]
Мы определим сложение \Ts преобразований по правилу
\begin{align*}
F_V+F_W&=F_{V\bigtriangleup W}\\
V\bigtriangleup W&=(V\cup W)\backslash(V\cap W)
\end{align*}
Очевидно, что
\[
F_\emptyset+F_V=F_V
\]
\[F_V+F_V=F_\emptyset\]
Следовательно, отображение $F_\emptyset$ является нулём относительно
сложения, а множество ${}^\star \Vector{M}$ является абелевой группой.}

\begin{theorem}
\label{theorem: Ts representation of the ring}
\Ts представление $f$
кольца $R$ на множестве $\Vector{M}$ определенно тогда и только
тогда, когда определены \Ts представления мультипликативной и аддитивной групп кольца $R$
и эти \Ts представления удовлетворяют соотношению
\[
f(a(b+c))=f(a)f(b)+f(a)f(c)
\]
\end{theorem}
\begin{proof}
Теорема следует из определения
\ref{definition: Tstar representation of algebra}.
\end{proof}

\begin{definition}
\label{definition: Tstar module}
$\Vector{M}$ - \AddIndex{$R\star$\Hyph модуль}{Rstar-module}
нaд кольцом $R$,
если $\Vector{M}$ - абелева группa и
определено \Ts представление кольца $R$.
\qed
\end{definition} 

Согласно нашим обозначениям $R\star$\hyph модуль -
это \AddIndex{левый модуль}{left module} и
\AddIndex{$\star R$\hyph модуль}{starR-module} -
это \AddIndex{правый модуль}{right module}.

Поле является частным случаем кольца. Поэтому векторное пространство над полем
имеет больше свойств чем модуль над кольцом.
Очень трудно, если вообще возможно,
распространить определения, работающие в векторном пространстве,
на модуль над произвольным кольцом.
Определение базиса и размерности векторного пространства тесно связаны с возможностью
найти решение линейного уравнения в кольце.
Свойства линейного уравнения в теле близки к свойствам
линейного уравнения в поле.
Поэтому мы надеемся что свойства векторного пространства над телом
близки к свойствам векторного пространства над полем.

\begin{theorem}
\label{theorem: effective Ts representation of the division ring}
\Ts представление тела $D$
\AddIndex{эффективно}{effective representation of division ring},
если эффективно \Ts представление мультипликативной группы тела $D$.
\end{theorem}
\begin{proof}
Пусть
\begin{equation}
f:D\rightarrow {}^\star M
\label{eq: Tstar representation of division ring}
\end{equation}
\Ts представление тела $D$. Если элементы $a$, $b$ мультипликативной группы
порождают одно и то \Ts преобразование, то
\begin{equation}
f(a)m=f(b)m
\label{eq: Tstar representation of division ring, 1}
\end{equation}
для любого $m\in M$. Выполняя преобразование $f(a^{-1})$ над обеими частями
равенства \EqRef{Tstar representation of division ring, 1}, мы получим
\[
m=f(a^{-1})(f(b)m)=f(a^{-1}b)m
\]
\end{proof}

Согласно замечанию
\ref{remark: notation for effective representation of algebra},
если представление тела эффективно, мы отождествляем элемент тела и соответствующее
ему \Ts преобразование.

\begin{definition}
\label{definition: Tstar vector space}
$\Vector V$ - \AddIndex{$D\star$\Hyph векторное пространство}{Dstar vector space}
нaд телом $D$,
если $\Vector V$ - абелева группa и
определено эффективное \Ts представление тела $D$.
\qed
\end{definition} 

\begin{theorem}
\label{theorem: definition of vector space}
Элементы $D\star$\Hyph векторного пространства $\Vector V$ удовлетворяют
соотношениям
\begin{itemize}
\item 
\AddIndex{закону ассоциативности}{associative law, Dstar vector space}
\begin{equation}
\label{eq: associative law, Dstar vector space}
(ab)\Vector{m}=a(b\Vector{m})
\end{equation}
\item 
\AddIndex{закону дистрибутивности}{distributive law, Dstar vector space}
\begin{align}
\label{eq: distributive law, Dstar vector space, 1}
a(\Vector{m}+\Vector{n})&=a\Vector{m}+a\Vector{n}\\
\label{eq: distributive law, Dstar vector space, 2}
(a+b)\Vector{m}&=a\Vector{m}+b\Vector{m}
\end{align}
\item 
\AddIndex{закону унитарности}{unitarity law, Dstar vector space}
\begin{equation}
\label{eq: unitarity law, Dstar vector space}
1\Vector{m}=\Vector{m}
\end{equation}
\end{itemize}
для любых $a, b \in D$, $\Vector{m}, \Vector{n} \in \Vector V$.
Мы будем называть \Ts представление
\AddIndex{$D\star$\Hyph произведением вектора на скаляр}{Dstar product of vector over scalar, vector space}.
\end{theorem}
\begin{proof}
Равенство \EqRef{distributive law, Dstar vector space, 1} следует
из утверждения, что \Ts преобразование $a$ является автоморфизмом абелевой группы.
Равенство \EqRef{distributive law, Dstar vector space, 2} следует
из утверждения, что \Ts представление является гомоморфизмом аддитивной группы
тела $D$.
Равенства \EqRef{associative law, Dstar vector space} и
\EqRef{unitarity law, Dstar vector space} следуют
из утверждения, что \Ts представление является ковариантным
\Ts представлением мультипликативной группы тела $D$.
\end{proof}

Согласно нашим обозначениям $D\star$\hyph векторное пространство -
это \AddIndex{левое векторное пространство}{left vector space} и
\AddIndex{$\star D$\hyph векторное пространство}{starD-vector space} -
это \AddIndex{правое векторное пространство}{right vector space}.

\begin{definition}
Пусть $\Vector V$ - $D\star$\hyph векторное пространство нaд телом $D$.
Множество векторов $\Vector{N}$ -
\AddIndex{подпространство $D\star$\hyph векторного пространства}
{subspace of Dstar vector space}
$\Vector V$, если
\ShowEq{subspace of Dstar vector space}
\qed
\end{definition}

\begin{example}
\label{example: matrices vector space}
Определим на множестве
\symb{D^m_n}1{matrices vector space}
$m\times n$
матриц над телом $D$
операцию сложения
\[
a+b=
\left(a_i^j\right)
+
\left(b_i^j\right)
=
\left(a_i^j+b_i^j\right)
\]
и умножения на скаляр
\[
da=
d\left(a_i^j\right)
=
\left(da_i^j\right)
\]
$a=0$ тогда и только тогда, когда $a_i^j=0$ для любых $i$, $j$.
Непосредственная проверка показывает, что
$D^m_n$ является $D\star$\hyph векторным пространством,
если произведение действует слева.
В противном случае $D^m_n$
- $\star D$\hyph векторное пространство.
Мы будем называть векторное пространство $D^m_n$
\AddIndex{$D\star$\hyph векторным пространством матриц}{matrices vector space}.
\qed
\end{example}

\section{Тип векторного пространства}
\label{section: vector space type}

Произведение вектора на скаляр асимметрично,
так как произведение определено для объектов разных множеств.
Однако различие между $D\star$\hyph\ и $\star D$\hyph векторным пространством появляется только тогда,
когда мы переходим к координатному представлению.
Говоря, векторное пространство является $D\star$\hyph\ или $\star D$\hyph, мы указываем,
с какой стороны, слева или справа, мы умножаем координаты
вектора на элементы тела.

\begin{definition}
Допустим $u$, $v$ - векторы $D\star$\hyph векторного пространства $\Vector V$. Мы будем
говорить, что вектор $w$ является
\AddIndex{$D\star$\hyph линейной комбинацией векторов}{linear composition of  vectors} $u$ и $v$,
если мы можем записать $w=au+bv$, где $a$ и $b$ - скаляры.
\qed
\end{definition}

Мы можем распространить понятие линейной комбинации на любое конечное семейство
векторов. Пользуясь обобщённым индексом для нумерации векторов, мы
можем представить семейство векторов в виде одномерной матрицы.
Мы пользуемся соглашением, что в заданном векторном пространстве мы представляем любое семейство
векторов либо в виде \subs строки, либо \sups строки.
Это представление
определяет характер записи линейной комбинации.
Рассматривая это представление в $D\star$- или $\star D$\hyph векторном пространстве, мы
получаем четыре разных модели векторного пространства.

Чтобы иметь возможность,
не меняя записи указать, является векторное пространство
$D\star$- или $\star D$\hyph векторным пространством, мы вводим новое обозначение.
Символ \symb{D\star}1{vector space type}\ называется \AddIndex{типом векторного пространства}{vector space type} и
означает, что мы изучаем $D\star$\hyph векторное пространство над телом $D$.
Операция умножения в типе векторного пространства указывает на матричную операцию, используемую в
линейной комбинации.

\begin{example}
Представим множество векторов
\ShowEq{sups row Vector A, 1}
\AddIndex{\drc векторного пространства}{drc vector space} $\Vector V$
в виде \sups строки
\ShowEq{sups row Vector A}
и множество скаляров
\ShowEq{subs row c, 1},
в виде \subs строки
\ShowEq{subs row c}
Тогда мы можем записать линейную комбинацию векторов $\pia$ в виде
\ShowEq{linear composition pVa}
Мы пользуемся записью \symb{{}_{D\RCstar}\Vector V}1{left RC vector space},
когда мы хотим сказать, что $\Vector V$ - \drc векторное пространство.
\qed
\end{example}

\begin{example}
Представим множество векторов
\ShowEq{subs row Vector A, 1}
\AddIndex{\dcr векторного пространства}{dcr vector space} $\Vector V$
в виде \subs строки
\ShowEq{subs row Vector A}
и множество скаляров
\ShowEq{sups row c, 1},
в виде \sups строки
\ShowEq{sups row c}
Тогда мы можем записать линейную комбинацию векторов $\bia$ в виде
\ShowEq{linear composition bVa}
Мы пользуемся записью \symb{{}_{D\CRstar}\Vector V}1{left CR vector space},
когда мы хотим сказать, что $\Vector V$ - \dcr векторное пространство.
\qed
\end{example}

\begin{example}
Представим множество векторов
\ShowEq{Vector A sups row, 1}
\AddIndex{\crd векторного пространства}{crd vector space} $\Vector V$
в виде \sups строки
\ShowEq{Vector A sups row}
и множество скаляров
\ShowEq{c subs row, 1},
в виде \subs строки
\ShowEq{c subs row}
Тогда мы можем записать линейную комбинацию векторов $\api$ в виде
\ShowEq{linear composition Vap}
Мы пользуемся записью \symb{\Vector V_{\CRstar D}}1{right CR vector space},
когда мы хотим сказать, что $\Vector V$ - \crd векторное пространство.
\qed
\end{example}

\begin{example}
Представим множество векторов
\ShowEq{Vector A subs row, 1}
\AddIndex{\rcd векторного пространства}{rcd vector space} $\Vector V$
в виде \subs строки
\ShowEq{Vector A subs row}
и множество скаляров
\ShowEq{c sups row, 1},
в виде \sups строки
\ShowEq{c sups row}
Тогда мы можем записать линейную комбинацию векторов $\abi$ в виде
\ShowEq{linear composition Vab}
Мы пользуемся записью \symb{\Vector V_{\RCstar D}}1{right RC vector space},
когда мы хотим сказать, что $\Vector V$ - \rcd векторное пространство.
\qed
\end{example}

\begin{remark}
\label{remark: left and right vector space notation}
Мы распространим на векторное пространство и его тип соглашение,
описанное в замечании
\xRef{0612.111}{remark: left and right matrix notation}.
Например, в выражении
\[A\RCstar B\RCstar v\lambda\]
мы выполняем операцию умножения слева направо. Это соответствует
\rcd векторному пространству. Однако мы можем выполнять операцию умножения
справа налево. В традиционной записи это выражение примет вид
\[\lambda v\CRstar B\CRstar A\]
и будет соответствовать \dcr векторному пространству. Аналогично, читая выражение
снизу вверх мы получим выражение
\[A\CRstar B\CRstar v\lambda\]
соответствующего \crd векторному пространству.
\qed
\end{remark}

\section{\texorpdfstring{$\RCstar D$}{rcD}-базис векторного пространства}
\label{section: Basis of Vector Space}

\begin{definition}
Векторы
\ShowEq{Vector A subs row, 1}
\rcd векторного пространства
$\Vector V$ \AddIndex{\rcd линейно независимы}
{linearly independent, vector space},
если $c=0$ следует из уравнения
\ShowEq{rcd linearly independent}
В противном случае, векторы $\Abi$
\AddIndex{\rcd линейно зависимы}{linearly dependent, vector space}.
\qed
\end{definition}

\begin{definition}
Множество векторов
\ShowEq{basis, vector space}
- \AddIndex{\rcd базис векторного пространства}{rcd basis, vector space},
если векторы $\Veb$ \rcd линейно независимы и добавление
любого вектора к этой системе
делает эту систему \rcd линейно зависимой.
\qed
\end{definition}

\begin{theorem}
\label{theorem: expansion relative basis, vector space}
Если $\Basis e$ - \rcd базис векторного пространства $\Vector V$,
то любой вектор $\Vector v\in \Vector V$
имеет одно и только одно разложение
\ShowEq{expansion relative basis, vector space}
относительно этого \rcd базиса.
\end{theorem}
\begin{proof}
Так как система векторов $\Veb$ является
максимальным множеством \rcd линейно независимых векторов,
система векторов
\ShowEq{expansion relative basis, vector space, 0}
- \drc линейно зависима и в уравнении
\ShowEq{expansion relative basis, vector space, 1}
по крайней мере $b$ отлично от $0$. Тогда равенство
\ShowEq{expansion relative basis, vector space, 2}
следует из \EqRef{expansion relative basis, vector space, 1}.
\EqRef{expansion relative basis, vector space} следует
из \EqRef{expansion relative basis, vector space, 2}.

Допустим мы имеем другое разложение
\ShowEq{expansion relative basis, vector space, 3}
Вычтя \EqRef{expansion relative basis, vector space}
из \EqRef{expansion relative basis, vector space, 3},
мы получим
\ShowEq{expansion relative basis, vector space, 4}
Так как векторы $\Veb$ \rcd линейно независимы, мы имеем
\[v'-v=0\]
\end{proof}

\begin{definition}
Мы будем называть матрицу
$v$ разложения \EqRef{expansion relative basis, vector space}
\AddIndex{координатной матрицей вектора $\Vector v$ в \rcd базисе $\Basis e$}
{coordinate matrix of vector in rcd basis}
и её элементы
\AddIndex{координатами вектора $\Vector v$ в \rcd базисе $\Basis e$}
{coordinates of vector in rcd basis}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: coordinate vector space}
Множество координат $a$ вектора $\Vector a$ в \rcd базисе $\Basis e$
порождают \rcd векторное пространство \symb{D^n}1{coordinate rcd vector space},
изоморфное \rcd векторному пространству $\Vector V$.
Это \rcd векторное пространство называется
\AddIndex{координатным \rcd векторным пространством}
{coordinate rcd vector space},
а изоморфизм
\AddIndex{координатным \rcd изоморфизмом}{coordinate rcd isomorphism}.
\end{theorem}
\begin{proof}
Допустим векторы $\Vector a$ и $\Vector b\in\Vector V$ имеют разложение
\ShowEq{coordinate vector space, 1}
в базисе $\Basis e$. Тогда
\ShowEq{coordinate vector space, 2}
для любого $m\in D$.
Таким образом, операции в векторном пространстве определены по координатно
\ShowEq{coordinate vector space, 3}
Это доказывает теорему.
\end{proof}

\begin{example}
\label{example: rcd vector space}
Пусть
\ShowEq{rcd vector space}
- \rcd базис векторного пространства $D^n$.
Координатная матрица
\ShowEq{rcd vector}
вектора $\Vector a$ в \rcd базисе $\Basis e$
называется \AddIndex{\rcd вектором}{rcd vector}.\footnote{\rcd вектор
является аналогом вектор\hyph столбца.
Мы можем называть его также $D\star$\Hyph вектор \sups строкой}
Мы будем называть векторное пространство
\symb{D^n}1{c rows rcd vector space}
\AddIndex{\rcd векторным пространством \sups строк}{sups rows rcd vector space}.

Пусть \subs строка
\ShowEq{subs row, vectors}
задаёт множество векторов.
Векторы $\Abj$ имеют разложение
\ShowEq{subs row, vectors, 1}
Если мы подставим координатные матрицы вектора $\Abj$ в
матрицу \EqRef{subs row, vectors}, мы получим матрицу
\ShowEq{subs row, vectors, 2}
Мы будем называть матрицу $A$
\AddIndex{координатной матрицей множества векторов}
{coordinate matrix of set of vectors, rcd vector space}
\ShowEq{Vector A sups row, 2}
в базисе $\Basis e$
и её элементы
\AddIndex{координатами множества векторов}
{coordinates of set of vectors, rcd vector space}
\ShowEq{Vector A sups row, 2}
в базисе $\Basis e$.

Мы будем представлять
\AddIndex{\rcd базис $\Basis f$ векторного пространства \sups строк}
{rcd basis, c rows vector space}
$D^n$
в форме \subs строки
\ShowEq{basis, c rows rcd vector space}
Мы будем говорить, что координатная матрица $f$ множества векторов
\ShowEq{basis, c rows rcd vector space, 1}
определяет координаты
\ShowEq{basis, c rows rcd vector space, 2}
базиса $\Basis f$ относительно базиса $\Basis e$.
\qed
\end{example}

\begin{example}
\label{example: drc vector space}
Пусть
\ShowEq{drc vector space}
- \drc базис векторного пространства $D_n$.
координатная матрица
\ShowEq{drc vector}
вектора $\Vector a$ в \drc базисе $\Basis e$
называется \AddIndex{\drc вектором}{drc vector}.\footnote{\drc вектор
является аналогом вектор\hyph строки.
Мы можем называть его также $D\star$\Hyph вектор \subs строкой}
Мы будем называть векторное пространство
\symb{D_n}1{r rows drc vector space}
\AddIndex{\drc векторным пространством \subs строк}{subs rows drc vector space}.

Пусть \sups строка
\ShowEq{sups row, vectors}
задаёт множество векторов.
Векторы $\piA$ имеют разложение
\ShowEq{sups row, vectors, 1}
Если мы подставим координатные матрицы вектора $\piA$ в
матрицу \EqRef{sups row, vectors}, мы получим матрицу
\ShowEq{sups row, vectors, 2}
Мы будем называть матрицу $A$
\AddIndex{координатной матрицей множества векторов}{coordinate matrix of set of vectors, dcr vector space}
$({}^i\Vector A,i\in M)$ в базисе $\Basis e$
и её элементы
\AddIndex{координатами множества векторов}{coordinates of set of vectors, dcr vector space}
$({}^i\Vector A,i\in M)$ в базисе $\Basis e$.

Мы будем представлять
\AddIndex{\drc базис $\Basis f$ векторного пространства \subs строк}
{drc basis, r rows vector space}
$D_n$
в форме \sups строки
\ShowEq{basis, r rows drc vector space}
Мы будем говорить, что координатная матрица $f$ множества векторов
\ShowEq{basis, r rows drc vector space, 1}
определяет координаты
\ShowEq{basis, r rows drc vector space, 2}
базиса $\Basis f$ относительно базиса $\Basis e$.
\qed
\end{example}

Так как мы линейную комбинацию выражаем с помощью матриц, мы можем
распространить принцип двойственности на теорию векторных пространств.
Мы можем записать принцип двойственности в одной из следующих форм

\begin{theorem}[принцип двойственности]
\label{theorem: duality principle, vector space}
Пусть $\mathfrak{A}$ - истинное утверждение о векторных пространствах.
Если мы заменим одновременно
\begin{itemize}
\item \drc вектор и \dcr вектор
\item \rcd вектор и \crd вектор
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}

\begin{theorem}[принцип двойственности]
\label{theorem: duality principle, vector space, quasideterminants}
Пусть $\mathfrak{A}$ - истинное утверждение о векторных пространствах.
Если мы одновременно заменим
\begin{itemize}
\item \drc вектор и \rcd вектор или \dcr вектор и \crd вектор
\item \RC квазидетерминант и \CR квазидетерминант
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}

\Input{Rcd.Morphism}

\section{Система \texorpdfstring{$\RCstar D$}{rcD}\hyph линейных уравнений}
\label{section: System of Linear Equations}

\begin{definition}
\label{definition: linear span, vector space}
Пусть $\Vector V$ - \rcd векторное пространство и
\ShowEq{rcd linear span}
- множество векторов.
\AddIndex{\rcd линейная оболочка в векторном пространстве}{linear span, vector space}
- это множество
\ShowEq{linear span, vector space}
векторов, \rcd линейно зависимых от векторов $\Abi$.
\qed
\end{definition}

\begin{theorem}
Пусть $\spanb$ - \rcd линейная оболочка в
векторном пространстве $\Vector V$.
Тогда $\spanb$
- подпространство векторного пространства $\Vector V$.
\end{theorem}
\begin{proof}
Предположим, что
\ShowEq{linear span, vector space, 1}
Согласно определению \ref{definition: linear span, vector space}
\ShowEq{linear span, vector space, 2}
Тогда
\ShowEq{linear span, vector space, 3}
Это доказывает утверждение.
\end{proof}

\begin{example}
Пусть $\Vector V$ - \rcd векторное пространство и
\subs строка
\ShowEq{rcd linear span, 0}
задаёт множество векторов.
Чтобы ответить на вопрос, или вектор
\ShowEq{rcd linear span, 1},
мы запишем линейное уравнение
\ShowEq{rcd linear span, 2}
где
\ShowEq{rcd linear span, 3}
\sups строка неизвестных коэффициентов разложения.
\ShowEq{rcd linear span, 4},
если уравнение \EqRef{rcd linear span, 2}
имеет решение.
Предположим, что
\ShowEq{rcd linear span, 5}
- \rcd базис.
Тогда векторы
\ShowEq{rcd linear span, 6}
имеют разложение
\ShowEq{rcd linear span, 7}
Если мы подставим \EqRef{rcd linear span, b}
и \EqRef{rcd linear span, ai}
в \EqRef{rcd linear span, 2}, мы получим
\ShowEq{rcd linear span, 8}
Применяя теорему \ref{theorem: expansion relative basis, vector space}
к \EqRef{rcd linear span, 8}, мы получим
\AddIndex{систему \rcd линейных уравнений}
{system of rcd linear equations}
\ShowEq{system of rcd linear equations}

Мы можем записать систему \rcd линейных уравнений
\EqRef{system of rcd linear equations} в одной из следующих форм
\ShowEq{star rows system of linear equations}
\qed
\end{example}

\begin{example}
Пусть $\Vector V$ - \drc векторное пространство и
\sups строка
\ShowEq{drc linear span, 0}
задаёт множество векторов.
Чтобы ответить на вопрос, или вектор
\ShowEq{drc linear span, 1},
мы запишем линейное уравнение
\ShowEq{drc linear span, 2}
где
\ShowEq{drc linear span, 3}
\subs строка неизвестных коэффициентов разложения.
\ShowEq{drc linear span, 4},
если уравнение \EqRef{drc linear span, 2}
имеет решение.
Предположим, что
\ShowEq{drc linear span, 5}
- \drc базис.
Тогда векторы
\ShowEq{drc linear span, 6}
имеют разложение
\ShowEq{drc linear span, 7}
Если мы подставим \EqRef{drc linear span, b}
и \EqRef{drc linear span, ai}
в \EqRef{drc linear span, 2}, мы получим
\ShowEq{drc linear span, 8}
Применяя теорему \ref{theorem: expansion relative basis, vector space}
к \EqRef{drc linear span, 8}, мы получим
\AddIndex{систему \drc линейных уравнений}
{system of drc linear equations}\footnote{Читая систему
\rcd линейных уравнений \EqRef{system of rcd linear equations} снизу вверх
и слева направо,
мы получим систему \dcr линейных уравнений
\EqRef{system of drc linear equations}.}
\ShowEq{system of drc linear equations}

Мы можем записать систему \drc линейных уравнений
\EqRef{system of drc linear equations} в одной из следующих форм
\ShowEq{star columns system of linear equations}
\qed
\end{example}

\begin{definition}
Если $n\times n$ матрица $A$ имеет \RC обратную матрицу,
мы будем называть такую матрицу
\AddIndex{\RC невырожденной матрицей}{RC nonsingular matrix}.
В противном случае, мы будем называть такую матрицу
\AddIndex{\RC вырожденной матрицей}{RC singular matrix}.
\qed
\end{definition}

\begin{definition}
Предположим, что $A$
- \RC невырожденная матрица. Мы будем называть соответствующую систему
\rcd линейных уравнений
\ShowEq{nonsingular system of linear equations}
\AddIndex{невырожденной системой \rcd линейных уравнений}
{nonsingular system of linear equations}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: nonsingular system of linear equations}
Решение невырожденной системы \rcd линейных уравнений
\EqRef{nonsingular system of linear equations} определено однозначно
и может быть записано в любой из следующих форм\footnote{Мы можем найти решение системы
\EqRef{nonsingular system of linear equations}
в теореме
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
Я повторяю это утверждение, так как я слегка изменил обозначения.
\label{footnote: nonsingular system of linear equations}}
\ShowEq{nonsingular system of linear equations, solution}
\end{theorem}
\begin{proof}
Умножая обе части равенства \EqRef{nonsingular system of linear equations}
слева на $A^{\RCInverse}$, мы получим
\EqRef{nonsingular system of linear equations, solution, matrix}.
Пользуясь определением
\xEqRef{0612.111}{eq: RC-quasideterminant definition},
мы получим \EqRef{nonsingular system of linear equations, solution, quasideterminant}.
Решение системы единственно в силу теоремы
\xEqRef{0612.111}{theorem: two products equal}.
\end{proof}

\section{Ранг матрицы}
\label{section: Rank of Matrix}

\begin{definition}
Мы будем называть матрицу\footnote{Мы
делаем следующие предположения в этом разделе
\begin{itemize}
\ShowEq{Rank of Matrix assumption 1}
\ShowEq{Rank of Matrix assumption 2}
- произвольная матрица.
\ShowEq{Rank of Matrix assumption 3 4}
\end{itemize}
\label{footnote: index assumption}}
$\SA T$ минором порядка $k$.
\qed
\end{definition}

\begin{definition}
Если минор $\SA T$ - \RC невырожденная матрица,
то мы будем говорить, что
\RC ранг матрицы $A$ не меньше, чем $k$.
\AddIndex{\RC ранг матрицы $A$}{rc-rank of matrix}
\ShowEq{rc-rank of matrix}
- это максимальное значение $k$.
Мы будем называть соответствующий минор \AddIndex{\RC главным минором}{RC-major minor}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: singular matrix and quasideterminant}
Пусть матрица $A$ - \RC вырожденная матрица и минор $\SA T$
- главный минор, тогда
\ShowEq{singular matrix and quasideterminant}
\end{theorem}
\begin{proof}
Чтобы понять, почему минор $\SATpr$
не имеет \RC обратной матрицы,\footnote{Естественно ожидать связь между \RC вырожденностью матрицы
и её \RC квазидетерминантом, подобную связи, известной в коммутативном случае.
Однако \RC квазидетерминант определён не всегда. Например, если \RC обратная матрица
имеет слишком много элементов, равных $0$. Как следует из этой теоремы, не определён \RC квазидетерминант
также в случае, когда \RC ранг матрицы меньше $n-1$.}
мы предположим, что он имеет \RC обратную матрицу
и запишем соответствующую систему
\xEqRef{0612.111}{eq: inverse minor, 11},
\xEqRef{0612.111}{eq: inverse minor, 12},
полагая $i=r$, $j=p$ и попробуем решить эту систему.
Положив
\ShowEq{singular matrix and quasideterminant, 0}
мы получим систему
\ShowEq{singular matrix and quasideterminant, 1}
Мы умножим \EqRef{singular matrix and quasideterminant, 1} на
$\Bf$
\ShowEq{singular matrix and quasideterminant, 3}
Теперь мы можем подставить \EqRef{singular matrix and quasideterminant, 3} в
\EqRef{singular matrix and quasideterminant, 2}
\ShowEq{singular matrix and quasideterminant, 4}
Из \EqRef{singular matrix and quasideterminant, 4} следует
\ShowEq{singular matrix and quasideterminant, 5}
Выражение в скобках является квазидетерминантом
$\Bq$.
Подставляя это выражение в \EqRef{singular matrix and quasideterminant, 5},
мы получим
\ShowEq{singular matrix and quasideterminant, 6}
Тем самым мы доказали, что квазидетерминант $\Bq$
определён и условие его обращения в $0$ необходимое и достаточное условие
вырожденности матрицы $B$. Теорема доказана в силу соглашения
\EqRef{singular matrix and quasideterminant, 0}.
\end{proof}

\begin{theorem}
\label{theorem: rc rank of matrix, subs-rows}
Предположим, что $A$ - матрица,
$$\RCA=k<m$$
и $\SA T$ - \RC главный минор.
Тогда \subs строка ${}^pA$ является
\drc линейной комбинацией \subs строк ${}^SA$.
\ShowEq{rc rank of matrix, subs-rows}
\end{theorem}
\begin{proof}
Если число \sups строк - $k$, то, полагая, что \subs строка ${}^pA$
- \drc линейная комбинация \EqRef{rc rank of matrix, subs-rows, 1}
\subs строк ${}^sA$ с коэффициентами $\pRs$,
мы получим систему \EqRef{rc rank of matrix, subs-rows, 2}.
Согласно теореме \ref{theorem: nonsingular system of linear equations}
эта система имеет единственное решение\footnote{Мы положим,
что неизвестные переменные здесь - это $x_s=\pRs$
\label{footnote: xs=rps}}
и оно нетривиально потому, что все \RC квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \sups строк больше чем $k$.
Пусть нам даны \subs строка ${}^pA$ и \sups строка $A_r$.
Согласно предположению минор
$\SATpr$ - \RC вырожденная матрица
и его \RC квазидетерминант
\ShowEq{rc rank of matrix, subs-rows, 3}
Согласно
\xEqRef{0612.111}{eq: quasideterminant, 1}
равенство \EqRef{rc rank of matrix, subs-rows, 3} имеет вид
\ShowEq{rc rank of matrix, subs-rows, 4}
Матрица
\ShowEq{rc rank of matrix, subs-rows, 5}
не зависят от $r$. Следовательно, для любых $r\in N\setminus T$
\ShowEq{rc rank of matrix, subs-rows, 6}

Из равенства
\ShowEq{rc rank of matrix, subs-rows, 7}
следует, что
\ShowEq{rc rank of matrix, subs-rows, 8}
Подставляя \EqRef{rc rank of matrix, subs-rows, 5}
в \EqRef{rc rank of matrix, subs-rows, 8}, мы получим
\ShowEq{rc rank of matrix, subs-rows, 9}
\EqRef{rc rank of matrix, subs-rows, 6} и \EqRef{rc rank of matrix, subs-rows, 9}
завершают доказательство.
\end{proof}

\begin{corollary}
\label{corollary:rc rank of matrix, subs-rows}
Предположим, что $A$ - матрица,
$\RCA=k<m$.
Тогда \subs строки матрицы \drc линейно зависимы.
\begin{equation}
\label{eq: rc rank of matrix, subs-rows drc linearly dependent}
\lambda\RCstar A=0
\end{equation}
\end{corollary}
\begin{proof}
Предположим, что \subs строка ${}^pA$ - \drc линейная комбинация
\EqRef{rc rank of matrix, subs-rows, 1}. Мы положим
\ShowEq{rc rank of matrix, subs-rows drc linearly dependent, 1}
и остальные
\ShowEq{rc rank of matrix, subs-rows drc linearly dependent, 2}
\end{proof}

\begin{theorem}
\label{theorem: rank of coordinate matrix}
Пусть
\ShowEq{rank of coordinate matrix}
семейство
\drc линейно независимых векторов. Тогда \RC ранг их
координатной матрицы равен $m$.
\end{theorem}
\begin{proof}
Согласно конструкции, изложенной в примере \ref{example: drc vector space},
координатная матрица семейства векторов $({}^i\Vector A)$ относительно базиса $\Basis e$
состоит из \subs строк, являющихся координатными матрицами векторов
${}^i\Vector A$ относительно базиса $\Basis e$. Поэтому \RC ранг
этой матрицы не может превышать $m$.

Допустим \RC ранг
координатной матрицы меньше $m$.
Согласно следствию \ref{corollary:rc rank of matrix, subs-rows}
\subs строки матрицы \drc линейно зависимы. Если мы умножим обе части равенства
\EqRef{rc rank of matrix, subs-rows drc linearly dependent} на
\sups строку $\Vector e$ 
и положим $c=\lambda\RCstar A$, то мы получим, что \drc линейная комбинация
\[
c\RCstar \Vector e=0
\]
векторов базиса равна $0$. Это противоречит утверждению, что векторы $\Vector e$ образуют
базис. Утверждение теоремы доказано.
\end{proof}

\begin{theorem}
\label{theorem: rc rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$$\RCA=k<n$$
и $\SA T$ - \RC главный минор.
Тогда \sups строка $A_r$ является
\rcd линейной композицией \sups строк $A_t$
\ShowEq{rc rank of matrix, sups-rows}
\end{theorem}
\begin{proof}
Если число \subs строк - $k$, то, полагая, что \sups строка $A_r$
- \rcd линейная комбинация \EqRef{rc rank of matrix, sups-rows, 1}
\sups строк $A_t$ с коэффициентами $\tRr$,
мы получим систему \EqRef{rc rank of matrix, sups-rows, 2}.
Согласно теореме \ref{theorem: nonsingular system of linear equations}
эта система имеет единственное решение\footnote{Мы положим,
что неизвестные переменные здесь - это ${}^tx=\tRr$
\label{footnote: xt=rtq}}
и оно нетривиально потому, что все \RC квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \subs строк больше, чем $k$.
Пусть нам даны \sups строка $A_r$ и \subs строка ${}^pA$.
Согласно предположению минор
$\SATpr$ - \RC вырожденная матрица
и его \RC квазидетерминант
\ShowEq{rc rank of matrix, sups-rows, 3}
Согласно
\xEqRef{0612.111}{eq: quasideterminant, 1}
\EqRef{rc rank of matrix, sups-rows, 3} имеет вид
\ShowEq{rc rank of matrix, sups-rows, 5}
Матрица
\ShowEq{rc rank of matrix, sups-rows, 6}
не зависит от $p$, Следовательно, для любых $p\in M\setminus S$
\ShowEq{rc rank of matrix, sups-rows, 7}

Из равенства
\ShowEq{rc rank of matrix, sups-rows, 8}
следует, что
\ShowEq{rc rank of matrix, sups-rows, 9}
Подставляя \EqRef{rc rank of matrix, sups-rows, 6}
в \EqRef{rc rank of matrix, sups-rows, 9}, мы получим
\ShowEq{rc rank of matrix, sups-rows, 10}
\EqRef{rc rank of matrix, sups-rows, 7}
и \EqRef{rc rank of matrix, sups-rows, 10}
завершают доказательство.
\end{proof}

\begin{corollary}
\label{corollary:rc rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$\RCA=k<m$.
Тогда \sups строки матрицы \rcd линейно зависимы.
\[
A\RCstar \lambda=0
\]
\end{corollary}
\begin{proof}
Предположим, что \sups строка $A_r$ - правая линейная комбинация
\EqRef{rc rank of matrix, sups-rows, 1}. Мы положим
\ShowEq{rc rank of matrix, sups-rows rcd linearly dependent, 1}
и остальные
\ShowEq{rc rank of matrix, sups-rows rcd linearly dependent, 2}
\end{proof}

Опираясь на теорему \xRef{0612.111}{theorem: duality principle, quasideterminants},
мы можем записать подобные утверждения для \CR ранга матрицы.

\begin{theorem}
\label{theorem: cr rank of matrix, subs-rows}
Предположим, что $A$ - матрица,
\ShowEq{cr-rank of matrix}
и ${}_TA^S$ - \CR главный минор.
Тогда \subs строка $A^p$ является
\crd линейной композицией \subs строк $A^s$
\ShowEq{cr rank of matrix, subs-rows}
\end{theorem}

\begin{corollary}
\label{corollary: cr rank of matrix, subs-rows}
Предположим, что $A$ - матрица,
$\CRRank A=k<m$.
Тогда \subs строки матрицы \crd линейно зависимы.
\[
A\CRstar\lambda=0
\]
\end{corollary}

\begin{theorem}
\label{theorem: cr rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$$\CRRank A=k<n$$
и ${}_TA^S$ - \CR главный минор.
Тогда \sups строка ${}_rA$ является
\dcr линейной композицией \sups строк ${}_tA$
\ShowEq{cr rank of matrix, sups-rows}
\end{theorem}

\begin{corollary}
\label{corollary: cr rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$\CRRank a=k<m$.
Тогда \sups строки матрицы \dcr линейно зависимы.
\ShowEq{cr rank of matrix, sups-rows, 1}
\end{corollary}

\section{Система \texorpdfstring{$\RCstar D$}{rcD}\hyph линейных уравнений}

\begin{definition}
Предположим, что\footref{footnote: index assumption}
$A$ - матрица системы \drc линейных уравнений
\EqRef{star columns system of linear equations}.
Мы будем называть матрицу
\ShowEq{extended matrix, system of drc linear equations}
\AddIndex{расширенной матрицей}{extended matrix, system of drc linear equations} этой системы.
\qed
\end{definition}

\begin{definition}
Предположим, что\footref{footnote: index assumption}
$A$ - матрица системы \rcd линейных уравнений
\EqRef{star rows system of linear equations}.
Мы будем называть матрицу
\ShowEq{extended matrix, system of rcd linear equations}
\AddIndex{расширенной матрицей}{extended matrix, system of rcd linear equations} этой системы.
\qed
\end{definition}

\begin{theorem}
\label{theorem: star rows system of linear equations}
Система \rcd линейных уравнений \EqRef{star rows system of linear equations}
имеет решение тогда и только тогда, когда
\ShowEq{star rows system of linear equations, rank}
\end{theorem}
\begin{proof}
Пусть $\SA T$ - \RC главный минор матрицы $A$.

Пусть система \rcd линейных уравнений \EqRef{star rows system of linear equations}
имеет решение
\ShowEq{star rows system of linear equations, solution}
Тогда
\ShowEq{star rows system of linear equations, 1}
Уравнение \EqRef{star rows system of linear equations, 1} может быть записано в форме
\ShowEq{star rows system of linear equations, 2}
Подставляя \EqRef{rc rank of matrix, sups-rows} в
\EqRef{star rows system of linear equations, 2}, мы получим
\ShowEq{star rows system of linear equations, 3}
Из \EqRef{star rows system of linear equations, 3} следует, что \subs строка
$b$ является \rcd линейной комбинацией \subs строк $A_T$
\ShowEq{star rows system of linear equations, 4}
Это эквивалентно уравнению \EqRef{star rows system of linear equations, rank}.

Нам осталось доказать, что существование решения \rcd системы линейных уравнений
\EqRef{star rows system of linear equations} следует из
\EqRef{star rows system of linear equations, rank}.
Истинность \EqRef{star rows system of linear equations, rank} означает, что
$\SA T$ - так же \RC главный минор расширенной матрицы.
Из теоремы \ref{theorem: rc rank of matrix, sups-rows} следует, что \subs строка $b$
является \rcd линейной композицией \subs строк $A_T$
\ShowEq{star rows system of linear equations, 5}
Полагая
\ShowEq{star rows system of linear equations, 6},
мы получим
\ShowEq{star rows system of linear equations, 7}
Следовательно, мы нашли, по крайней мере, одно решение системы \rcd линейных уравнений
\EqRef{star rows system of linear equations}.
\end{proof}

\begin{theorem}
\label{theorem: star rows system of linear equations, solution}
Предположим, что \EqRef{star rows system of linear equations}
- система \rcd линейных уравнений,
удовлетворяющих \EqRef{star rows system of linear equations, rank}.
Если $\RCA=k\le m$,
то решение системы зависит
от произвольных значений $m-k$ переменных, не включённых в \RC главный минор.
\end{theorem}
\begin{proof}
Пусть $\SA T$ - \RC главный минор матрицы $a$.
Предположим, что
\ShowEq{star rows system of linear equations, reduce, 1}
уравнение с номером $p$.
Применяя теорему \ref{theorem: rc rank of matrix, subs-rows}
к расширенной матрице \EqRef{extended matrix, system of drc linear equations}, мы получим
\ShowEq{star rows system of linear equations, reduce}
Подставляя \EqRef{star rows system of linear equations, reduce, 2}
и \EqRef{star rows system of linear equations, reduce, 3}
в \EqRef{star rows system of linear equations, reduce, 1}, мы получим
\ShowEq{star rows system of linear equations, reduce, 4}
\EqRef{star rows system of linear equations, reduce, 4} означает, что
мы можем исключить уравнение \EqRef{star rows system of linear equations, reduce, 1}
из системы \EqRef{star rows system of linear equations}
и новая система эквивалентна старой.
Следовательно, число уравнений может быть уменьшено до $k$.

В этом случае
у нас есть два варианта. Если число переменных также равно $k$, то
согласно теореме \ref{theorem: nonsingular system of linear equations} система имеет единственное решение
\EqRef{nonsingular system of linear equations, solution, quasideterminant}.
Если число переменных $m>k$, то мы можем передвинуть $m-k$ переменных, которые не
включены в \RC главный минор в правой части.
Присваивая произвольные значения этим переменным, мы определяем значение
правой части и для этого значения мы получим единственное решение
согласно теореме \ref{theorem: nonsingular system of linear equations}.
\end{proof}

\begin{corollary}
\label{corollary:  nonsingular rows system of linear equations}
Система \rcd линейных уравнений \EqRef{star rows system of linear equations}
имеет единственное решение тогда и только тогда, когда
её матрица невырожденная.
\qed
\end{corollary}

\begin{theorem}
\label{theorem: Solutions homogenous system of linear equations}
Решения однородной системы \rcd линейных уравнений
\ShowEq{homogenous system of linear equations}
порождают \rcd векторное пространство.
\end{theorem}
\begin{proof}
Пусть $\Vector{X}$ - множество решений системы \rcd линейных уравнений
\EqRef{homogenous system of linear equations}.
Предположим, что
\ShowEq{homogenous system of linear equations x}
и
\ShowEq{homogenous system of linear equations y}
Тогда \[x^a\ _aa^b=0\] \[y^a\ _aa^b=0\]
Следовательно,
\ShowEq{homogenous system of linear equations x+y}
Таким же образом мы видим
\ShowEq{homogenous system of linear equations xb}
Согласно определению \ref{definition: Tstar vector space}
$\Vector{X}$ является \rcd векторным пространством.
\end{proof}

\section{Невырожденная матрица}

Предположим, что нам дана $n\times n$ матрица $A$.
Следствия \ref{corollary:rc rank of matrix, subs-rows}
и \ref{corollary:rc rank of matrix, sups-rows}
говорят нам, что если $\RCA<n$,
то \subs строки \drc линейно зависимы
и \sups строки \rcd линейно зависимы.\footnote{Это
утверждение похоже на утверждение
\citeBib{q-alg-9705026}-\href{http://arxiv.org/PS_cache/q-alg/pdf/9705/9705026.pdf\#Page=6}{1.2.5}.}

\begin{theorem}
\label{theorem: rc rank, sups rows}
Пусть $A$ - $n\times n$ матрица
и \sups строка $A_r$ - \rcd линейная комбинация других \sups строк.
Тогда $\RCA<n$.
\end{theorem}
\begin{proof}
Утверждение, что \sups строка $A_r$ является \rcd линейной комбинацией других \sups строк,
означает, что система \rcd линейных уравнений
\ShowEq{rc rank, sups rows}
имеет, по крайней мере, одно решение.
Согласно теореме \ref{theorem: star rows system of linear equations}
\ShowEq{rc rank, sups rows 1}
Так как число \sups строк меньше, чем $n$, то
\ShowEq{rc rank, sups rows 2}
\end{proof}

\begin{theorem}
\label{theorem: rc rank, subs rows}
Пусть $A$ - $n\times n$ матрица
и \subs строка ${}^pA$ - \drc линейная комбинация других \subs строк.
Тогда $\RCA<n$.
\end{theorem}
\begin{proof}
Доказательство утверждения похоже на доказательство теоремы
\ref{theorem: rc rank, sups rows}
\end{proof}

\begin{theorem}
Предположим, что $A$ и $B$ - $n\times n$ матрицы и
\begin{equation}
\label{eq: RC product singular, 1}
C=A\RCstar B
\end{equation}
$C$ - \RC вырожденная матрица тогда и только тогда, когда
либо матрица $A$, либо матрица $B$ - \RC вырожденная матрица.
\end{theorem}
\begin{proof}
Предположим, что матрица $B$ - \RC вырожденная.
Согласно теореме \ref{theorem: rc rank of matrix, sups-rows}
\sups строки матрицы $B$
\rcd линейно зависимы. Следовательно,
\ShowEq{RC product singular, 2}
где $\lambda\ne 0$. Из
\EqRef{RC product singular, 1}
и \EqRef{RC product singular, 2} следует, что
\ShowEq{RC product singular, 3}
Согласно теореме \ref{theorem: rc rank, sups rows} матрица $C$
является \RC вырожденной.

Предположим, что матрица $B$ - не \RC вырожденная, но матрица $A$ - \RC вырожденная.
Согласно теореме \ref{theorem: rc rank of matrix, subs-rows}
\sups строки матрицы $A$
\rcd линейно зависимы. Следовательно,
\ShowEq{RC product singular, 4}
где $\mu\ne 0$. Согласно
теореме \ref{theorem: nonsingular system of linear equations} система
\ShowEq{RC product singular, 5}
имеет единственное решение, где $\lambda\ne 0$.
Следовательно,
\ShowEq{RC product singular, 6}
Согласно теореме \ref{theorem: rc rank, sups rows} матрица $C$ является \RC вырожденной.

Предположим, что матрица $C$ - \RC вырожденная матрица.
Согласно теореме \ref{theorem: rc rank of matrix, subs-rows}
\subs строки матрицы $C$
\rcd линейно зависимы. Следовательно,
\ShowEq{RC product singular, 7}
где $\lambda\ne 0$.
Из \EqRef{RC product singular, 1}
и \EqRef{RC product singular, 7} следует, что
\ShowEq{RC product singular, 8}
Если 
\ShowEq{RC product singular, 9}
выполнено, то матрица $B$ - \RC вырожденная. Предположим, что
матрица $B$ не \RC вырожденная. Положим
\ShowEq{RC product singular, 10}
где $\mu\ne 0$. Тогда
\ShowEq{RC product singular, 11}
Из \EqRef{RC product singular, 11} следует, что
матрица $A$ - \RC вырожденная.
\end{proof}

Опираясь на теорему \xRef{0612.111}{theorem: duality principle, quasideterminants},
мы можем записать подобные утверждения для \dcr линейной комбинации \subs строк
или \crd линейной комбинации \sups строк и \CR квазидетерминанта.

\begin{theorem}
\label{theorem: cr rank, rows}
Пусть $A$ - $n\times n$ матрица
и \sups строка ${}_rA$ - \crd линейная комбинация других \sups строк.
Тогда $\CRRank  A<n$.
\end{theorem}

\begin{theorem}
\label{theorem: cr rank, columns}
Пусть $A$ - $n\times n$ матрица
и \subs строка $A^p$ - \dcr линейная комбинация других \subs строк.
Тогда $\CRRank  A<n$.
\end{theorem}

\begin{theorem}
Предположим, что $A$ и $B$ - $n\times n$ матрицы и
$C=A\CRstar B$. $C$ - \CR вырожденная матрица тогда и только тогда, когда
либо матрица $A$, либо матрица $B$ - \CR вырожденная матрица.
\end{theorem}

\begin{definition}
\AddIndex{\RC матричная группа}{rc-matrix group}
\symb{\RCGL nD}1{rc-matrix group} - это группа
\RC невырожденных матриц, гле мы определяем
\RC произведение матриц
\xEqRef{0612.111}{eq: rc-product of matrices}
и \RC обратную матрица
$A^{\CRInverse}$.
\qed
\end{definition}

\begin{definition}
\AddIndex{\CR матричная группа}{cr-matrix group}
\symb{\CRGL nD}1{cr-matrix group} - это группа
\CR невырожденных матриц
где мы определяем
\CR произведение матриц
\xEqRef{0612.111}{eq: cr-product of matrices}
и \CR обратную матрицу
$A^{\CRInverse}$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: CR RC singular matrix}
\[
\RCGL nD\ne \CRGL nD
\]
\end{theorem}
\begin{remark}
Из теоремы
\xEqRef{0612.111}{theorem: RC-inverse matrix, delta}
следует, что
существуют матрицы, которые \CR невырожденны и \RC невырожденны.
Теорема \ref{theorem: CR RC singular matrix} означает, что множества
\CR невырожденных матриц и \RC невырожденных матриц
не совпадают. Например,
существует такая \RC невырожденная матрица, которая
\CR вырожденная матрица.
\qed
\end{remark}
\begin{proof}
Это утверждение достаточно доказать для $n=2$.
Предположим, что каждая \CR вырожденная матрица
\ShowEq{RC-singular matrix, 1}
является \RC вырожденной матрицей.
Из теоремы \ref{theorem: rc rank of matrix, sups-rows} и
теоремы \ref{theorem: rc rank of matrix, sups-rows} следует, что
\RC вырожденная матрица удовлетворяет условию
\ShowEq{RC, a22, 1}
Если мы подставим \EqRef{RC, column, 1 2, 1 1}
в \EqRef{RC, row, 2 2, 1 2}, мы получим
\ShowEq{RC, a22, 2}
$b$ и $c$ - произвольные элементы тела $D$ и \RC вырожденная матрица
\EqRef{RC-singular matrix, 1} имеет вид ($d={}^1A_1$)
\ShowEq{RC-singular matrix, 2}
Подобным образом мы можем показать, что \CR вырожденная матрица
имеет вид
\ShowEq{CR-singular matrix, 2}
Из предположения следует, что \EqRef{CR-singular matrix, 2}
и \EqRef{RC-singular matrix, 2} представляют одну и ту же матрицу.
Сравнивая \EqRef{CR-singular matrix, 2}
и \EqRef{RC-singular matrix, 2}, мы получим, что
для любых $d,c\in D$ существует такое $c'\in D$, которое не зависит от $d$ и
удовлетворяет уравнению
\[d c=c'd\]
Это противоречит утверждению, что $D$ - тело.
\end{proof}

\begin{example}
В случае тела кватернионов мы положим $b=1+k$, $c=j$, $d=k$.
Тогда мы имеем
\ShowEq{example rc singular matrix}

Система \rcd линейных уравнений
\ShowEq{example rc singular matrix, rcd}
имеет \RC вырожденную матрицу.
Мы можем записать систему \rcd линейных уравнений
\EqRef{example rc singular matrix, rcd} в виде
\ShowEq{example rc singular matrix, rcd 1}

Система \crd линейных уравнений
\ShowEq{example rc singular matrix, crd}
имеет \CR невырожденную матрицу.
Мы можем записать систему \crd линейных уравнений
\EqRef{example rc singular matrix, crd} в виде
\ShowEq{example rc singular matrix, crd 1}

Система \drc линейных уравнений
\ShowEq{example rc singular matrix, drc}
имеет \RC вырожденную матрицу.
Мы можем записать систему \drc линейных уравнений
\EqRef{example rc singular matrix, drc} в виде
\ShowEq{example rc singular matrix, drc 1}

Система \dcr линейных уравнений
\ShowEq{example rc singular matrix, dcr}
имеет \CR невырожденную матрицу.
Мы можем записать систему \dcr линейных уравнений
\EqRef{example rc singular matrix, dcr} в виде
\ShowEq{example rc singular matrix, dcr 1}
\qed
\end{example}

\section{Размерность \texorpdfstring{$\RCstar D$}{rcD}\hyph векторного пространства}
\label{section: Dimension of Vector Space}

\begin{theorem}
\label{theorem: basis of vector space}
Пусть $\Vector V$ - \rcd векторное пространство. Предположим, что $\Vector V$ имеет
\rcd базисы
\ShowEq{basis e of V}
и
\ShowEq{basis g of V}
Если $|I|$ и $|J|$ - конечные числа, то $|I|=|J|$.
%Если $|S|$ is конечные число, то $|J|$ is конечные число и $|I|=|J|$.
\end{theorem}
\begin{proof}
Предположим, что $|I|=m$ и $|J|=n$. Предположим, что
\begin{equation}
m<n
\label{eq: basis of vector space, 0}
\end{equation}
Так как $\Basis e$ - \rcd базис, любой вектор
\ShowEq{basis g of V 1}
имеет разложение
\ShowEq{basis g of V 2}
Так как $\Basis{g}$ - \rcd базис
\ShowEq{basis g of V 3}
следует из
\ShowEq{basis g of V 4}
Так как $\Basis e$ - \rcd базис, мы получим
\ShowEq{basis g of V 5}
Согласно \EqRef{basis of vector space, 0}
$\RCA\le m$ и система \EqRef{basis g of V 5}
имеет больше переменных, чем уравнений. Согласно
теорема \ref{theorem: star rows system of linear equations, solution}
$\lambda\ne 0$. Это противоречит
утверждению \EqRef{basis g of V 3}. 
Следовательно, утверждение $m<n$ неверно.

Таким же образом мы можем доказать, что утверждение $n<m$ неверно.
Это завершает доказательство теоремы.
\end{proof}

\begin{definition}
Мы будем называть
\AddIndex{размерностью \rcd векторного пространства}{dimension of vector space}
число векторов в базисе
\qed
\end{definition}

\begin{theorem}
\label{theorem: coordinate matrix of basis}
Координатная матрица \rcd базиса $\Basis{g}$ относительно \rcd базиса $\Basis e$
векторного пространства $\Vector V$ является \RC невырожденной матрицей.
\end{theorem}
\begin{proof}
Согласно лемме \ref{theorem: rank of coordinate matrix}
\rcd ранг координатной матрицы базиса $\Basis{g}$ относительно базиса $\Basis e$
равен размерности векторного пространства, откуда следует утверждение теоремы.
\end{proof}

\begin{definition}
Мы будем называть взаимно однозначное отображение $\Vector A:\Vector V\rightarrow \Vector W$ 
\AddIndex{\rcd изоморфизмом векторных пространств}{isomorphism of vector spaces},
если это отображение - \rcd линейное отображение
векторных пространств.
\qed
\end{definition}

\begin{definition}
\AddIndex{\rcd автоморфизм векторного пространства}{automorphism of vector space}
$\Vector V$ - это \rcd изоморфизм $\Vector A:\Vector V\rightarrow \Vector V$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: automorphism of vector space}
Предположим, что $\Basis f$ - \rcd базис в векторном пространстве $\Vector V$.
Тогда любой \rcd автоморфизм $\Vector A$ векторного пространства
$\Vector V$ имеет вид
\ShowEq{automorphism, vector space}
где $A$ - \RC невырожденная матрица.
\end{theorem}
\begin{proof}
\EqRef{automorphism, vector space} следует из
теоремы \ref{theorem: rcd linear map of rcd vector space}.
Так как $\Vector A$ - изоморфизм, то для каждого вектора $\Vector v'$ существует единственный вектор $\Vector v$ такой,
что $\Vector v'=\Vector v\RCstar \Vector A$.
Следовательно, система \rcd линейных уравнений \EqRef{automorphism, vector space}
имеет единственное решение. Согласно следствию \ref{corollary: nonsingular rows system of linear equations}
матрица $A$ невырожденна.
\end{proof}

\begin{theorem}
\label{theorem: Automorphisms of vector space form a group}
Автоморфизмы \rcd векторного пространства порождают группу $\RCGL nD$.
\end{theorem}
\begin{proof}
Если даны два автоморфизма $\Vector A$ и $\Vector B$, то мы можем записать
\ShowEq{Automorphisms of vector space}
Следовательно, результирующий автоморфизм имеет матрицу $A\RCstar B$.
\end{proof}

